Learning Optimal Representations with the Decodable Information Bottleneck

We address the question of characterizing and finding optimal representations for supervised learning. Traditionally, this question has been tackled using the Information Bottleneck, which compresses the inputs while retaining information about the targets, in a decoder-agnostic fashion. In machine learning, however, our goal is not compression but rather generalization, which is intimately linked to the predictive family or decoder of interest (e.g. linear classifier). We propose the Decodable Information Bottleneck (DIB) that considers information retention and compression from the perspective of the desired predictive family. As a result, DIB gives rise to representations that are optimal in terms of expected test performance and can be estimated with guarantees. Empirically, we show that the framework can be used to enforce a small generalization gap on downstream classifiers and to predict the generalization ability of neural networks.

==> appendices/algorithm.tex <==
\label{appx:algorithm}

==> appendices/proof_min_old.tex <==
\subsection{$\V$-Minimality}
\ydnote{Keep for Arxive?}

In this section we will formalize all the necessary tools to understand the two following subsections about $\V$-minimality.
We will formalize the necessary definitions and then prove lemmas that will be useful.

\subsubsection{Definitions}
\label{appx:formal_definitions}

First, let us review the notion of $\rv Y$ decomposition of $\rv X$.

\begin{restatable}{definition}{decomposition}\label{def:decomposition}
Let $\mathcal{X}_y \defeq \{ x \in \mathcal{X} \ | \ t(x)=y \}$ be the examples labeled with $y$, and
$\mathcal{T}_y \defeq \{ t' \ | \ t' : \mathcal{X}_y \to \mathcal{Y} \}$ be all possible labeling of $\mathcal{X}_y$. 
The $y$ decomposition of $\rv X$ is 
\[
\mathrm{Dec}(\rv X, y) \defeq \{ \rv N \ | \ \exists t' \in \mathcal{T}_y \ s.t. \ P_{\rv N|y} = t'_{*}(P_{\rv X|y}) \}
\]
where $t'_{*}(P_{\rv X|y})$ is the push forward of $P_{\rv X|y}$ by $t'$.
\end{restatable}


In the main text we only defined $\V$-minimal $\V$-sufficient, but we can also define a similar notion with respect to different functional families.

\begin{restatable}{definition}{GminVsuf}\label{def:GminVsuf}
A representation $\rv Z$ is $\mathcal{G}$-minimal and  $\V$-sufficient if $\rv Z \in  \arg \min_{\rv Z \in \Qsuff{}} \op{I_\mathcal{G}}{\rv Z \rightarrow \decxY{} }$.
\end{restatable}

Now let us formalize the notion of empirical risk minimizer (ERM).

\begin{restatable}{definition}{ERM}\label{def:ERM}
Let $\sampleD{}$ be a sampled dataset.
A predictor $\hat{f}^* \in \V$ is an empirical risk minimizer (ERM) using $\rv Z$ t.v.i. $\mathcal{Z}$  for $\mathcal{D}$ if 
\[
\eqCH{\hat{f}^*}{Y}{Z}{D} = \eCHF{Y}{Z}{D}
\]
We denote the set of ERMs as $\hat{\V}^*(\mathcal{D}, \rv Z)$.
\end{restatable}


\subsubsection{Lemmas}
\label{appx:proof_lemmas}


In this subsection we will prove a collection of lemmas that are useful for the two following sections that prove \cref{theo:opt_qmin} and \cref{prop:Vminsuff}.
Note that these lemmas use the three additional assumptions discussed in the second part of \cref{sec:appx_assumptions}.


For all $\V$-sufficient representations the best achievable test loss is always zero.




If the representation is $\V$-sufficient then it can be partitioned by $\mathcal{Y}$.
I.e. the supports of  each $\rv Z_y$ are non-overlapping.

\begin{restatable}{lemma}{VsuffSupp}\label{lemma:VsuffSupp}
$\rv Z \in \Qsuff{} \implies$ $\mathrm{supp}(P_{\rv Z | y}) \cap \mathrm{supp}(P_{\rv Z | y'}) = \varnothing$, $\forall y\neq y', \ y,y' \in \mathcal{Y}$.
\end{restatable}
\begin{proof}
Let us prove it by contrapositive. 
Namely, we will show $\mathrm{supp}(P_{\rv Z | y}) \cap \mathrm{supp}(P_{\rv Z | y'}) \neq \varnothing \implies \rv Z \not \in \Qsuff{}$.
$\mathrm{supp}(P_{\rv Z | y}) \cap \mathrm{supp}(P_{\rv Z | y'}) \neq \varnothing$ implies that $\exists y \neq y' \in \mathcal{Y}, \exists z \in \mathcal{Z}$ s.t. $P_{\rv Z | \rv Y}(z|y')  \neq 0$ and $P_{\rv Z | \rv Y}(z|y) \neq 0$.
Using Bayes rule, that means $P_{\rv Y | \rv Z}(y'|z)   \neq 0$ and $P_{\rv Y | \rv Z}(y|z)  \neq 0$ so $\nexists y \in \mathcal{Y}$ s.t. $P_{\rv Y | \rv Z}(y'|z) =  1$.
Due to the finite sample space assumption, this implies $0 < \op{H}{\rv Y \cond \rv Z}  = \CHU{Y}{Z}  \leq \CHF{Y}{Z} $. 
From \cref{lemma:perfecttest} we conclude that $\rv Z \not \in \Qsuff{}$ as desired.
\end{proof}

If the representation is $\V$-sufficient then there always exists at least one predictor that is optimal for training and for testing.

\begin{restatable}{lemma}{existperfect}\label{lemma:existperfect}
$\forall \family{}$, $\forall \rv Z \in \Qsuff{}$ there exists $ f \in \family{}$ s.t. $\forall \mathcal{D} \sim P_{\rv Z \times \rv Y}^N $, $\qCHF{Y}{z}=\CHF{Y}{z}=\eqCHF{Y}{z}{D}=\eCHF{Y}{z}{D}=0$
\end{restatable}


\begin{proof}
From \cref{lemma:perfecttest} we know that $\forall Z \in \Qsuff{}$ we have $\CHF{Y}{Z}=0$.
Select any $\rv Z \in \Qsuff{}$ and let $f \in \family{}$ be one of the optimal predictor $\qCHF{Y}{Z}=0$. 
As $\qCHF{Y}{Z}$ is an expectation of a non-negative discrete r.v., it is equal to zero if and only if  $\forall z \in \mathrm{supp}(\rv Z), \ \forall y \in \mathrm{supp}(\rv Y)$  we have $\log f[z](y)=0$.
$\eqCHF{Y}{Z}{D}$ is also a weighted average (discrete expectation) of $\log f[z](y)=0$ over a subset of the previous support $\hat{z} \in \mathrm{supp}(\hrv Z) \subseteqq \mathrm{supp}(\rv Z), \ \forall \hat{y} \in \mathrm{supp}(\hrv Y) \subseteqq \mathrm{supp}(\rv Y)$ so we conclude that $\eqCHF{Y}{Z}{D}=0$.
We thus found a classifier that reaches zero loss, so $\eCHF{Y}{Z}{D}=0$ (infimum and non negativity of log loss).
Putting all together, $\forall Z \in \Qsuff{}$ we have $\CHF{Y}{Z}=\eCHF{Y}{Z}{D}=\qCHF{Y}{Z}=\eqCHF{Y}{Z}{D}=0$ as desired.
\end{proof}



A representation is $\V$-minimal $\V$-sufficient if and only if it has no $\V$-information with any of the terms in the $\rv Y$ decomposition of $\rv X$.

\begin{restatable}{lemma}{zeroVminimal}\label{lemma:zeroVminimal}
$\forall \rv Z \in \Qsmin{} \iff \rv Z \in \Qsuff{}$ and $\forall y \in \mathcal{Y}, \forall \rv N \in \decxy{}$ we have $\DIF{N}{Z_y}=0$. 
\end{restatable}

\begin{proof} $ $ \\
($\impliedby$) Due to the non negativity of $\V$-information, we have $\forall \rv Z' \in \Qsuff{}$,  $0=\DIF{N}{Z_y} \leq \DIF{N}{Z'_y} $ so $\rv Z$ reaches the minimal achievable value in each term and thus also on their expectation $\DIFxzCy{}=0$. We thus conclude that $\rv Z \in \Qsmin{} \defeq \arg \min_{\rv Z \in \Qsuff{}} \DIFxzCy{}$.

($\implies$) 
Let us show that there is at least one $\rv Z \in \Qsmin{}$ s.t. $\forall y \in \mathcal{Y}, \forall \rv N \in \decxy{}, \ \DIF{N}{Z_y}=0 $, from which we will conclude that they all have to in order to minimize $\DIFxzCy{}$.
Note that $P_{\rv Z_y^* \cond \rv X_y}(z_y|x_y) = \frac{1}{|\preimage{f}{t(x_y)}|} = \frac{1}{|\preimage{f}{y}|} = P_{\rv Z_y^*}(z_y)$, where the last equality comes from the fact that $z_y$ is associated with a single label $y$.
An other way of saying it, is that $\rv X_y - y - \rv Z_y$ forms a Markov Chain, but $y$ is a constant.
We thus conclude $\rv Z_y^* \perp \rv X_y$, and because $\rv N = t'( \rv X_y)$ we also have $\rv Z_y^* \perp \rv N$, $\forall \rv N \in \decxy{}$. What we said holds $\forall y \in \mathcal{Y}$. And due to the the independence property of $\V$-information, we have $\DIF{N}{Z_y}=0$ as desired.
As we found one $\rv Z^* \in \Qsmin{}$ s.t. this is true, it must be for all $\rv Z \in \Qsmin{}$.
Indeed, due to the  positivity property it is the only way of reaching the minimal $\DIFxzCy{}=0$.
\end{proof}

Universal sufficient representation corresponds to the subset of sufficient representations that t.v.i. in the domain of predictors in $\universal{}$.

\begin{restatable}[Recoverability of sufficiency]{lemma}{recsuff}\label{prop:recsuff}
 Let $\universal{} = \PYZ{}$ be the universal family, then  $\Usuff{} = \suff{} \cap \mathcal{Z}$
\end{restatable}
\proof{
Let us denote $\Omega = \cup \mathcal{Z}$ as the set of all possible finite sample spaces.
We know that,  $\DI{\universal{}}{Y}{Z} = \MI{Y}{Z}$ so $\arg \min_{\rv Z \in \mathcal{Z}} \DI{\universal{}}{Y}{Z} = \arg \min_{\rv Z \in \mathcal{Z}} \MI{Y}{Z}$. Let us suppose that $\suff{} \cap \mathcal{Z}$ is non empty we have $\suff{} \cap \mathcal{Z} = ( \arg  \min_{\rv Z \in \Omega} \MI{Y}{Z} ) \cap \mathcal{Z}  =  \arg \min_{\rv Z \in \mathcal{Z}} \MI{Y}{Z} = \Usuff{}$ as desired.
To show that $\suff{} \cap \mathcal{Z}$ is indeed non empty, notice that one can always learn the sufficient representation $ \rv Z =\rv Y $  due to the assumption $|\mathcal{Y}| \leq |\mathcal{Z}|$ (when $|\mathcal{Y}| < |\mathcal{Z}|$, restrict the support to $\mathcal{Y}$) and the determinism of $\rv Y$.
}

Let us characterize the set of minimal sufficient representations in terms of independence.

\begin{restatable}[Characterization of Minimal Sufficient Representations]{lemma}{charminsuff}\label{prop:charminsuff}
Suppose $\rv Y $ is a deterministic function of $\rv Y = g(\rv X)$ then the set of minimal sufficient representations correspond to  $\smin{} = \{ \rv Z \in \suff{} | \ \ \rv Z \perp \rv X | \rv Y  \ \}$
\end{restatable}
\proof{
\begin{align*}
\smin{} &\defeq \arg \min_{Z \in \suff{}} \MI{X}{Z} \\
&= \arg \min_{Z \in \suff{}} \MI{X,g(\rv X)}{Z} & \text{Inv. bijections} \\
&= \arg \min_{Z \in \suff{}} \MI{X,\rv Y}{Z} & \text{Det. Labels} \\
&= \arg \min_{Z \in \suff{}} \op{I}{\rv X; \rv Z | \rv Y} + \MI{Z}{Y}   & \text{Chain Rule} \\
&= \arg \min_{Z \in \suff{}} \op{I}{\rv X; \rv Z | \rv Y}   & \text{Sufficiency} 
\end{align*}
Where the second line used the fact that $f(\rv X) = (\rv X, g(\rv X))$ is a bijection.
Notice that $\op{I}{\rv Y; \rv Z | \rv Y} \geq 0$ and we know that it can reach zero, for example with $\rv Z = \rv Y$ (which is sufficient).
So $\smin{} = \{ \rv Z \in \suff{} | \op{I}{\rv Y; \rv Z | \rv Y} = 0\} = \{ \rv Z \in \suff{} | \ \  \rv Z \perp \rv X | \rv Y  \ \}$ which concludes the proof.
}

Similarly, let us characterize the set of $\universal{}$-minimal $\universal{}$-sufficient representations in terms of independence.

\begin{restatable}[Characterization of $\universal{}$-Minimal $\universal{}$-Sufficient Representations]{lemma}{charUminUsuff}\label{prop:charUminUsuff}
Suppose $\rv Y $ is a deterministic function of $\rv Y = g(\rv X)$ then the set of minimal sufficient representations correspond to  $\Usmin{} = \{ \rv Z \in \Usuff{} | \ \forall y \in \mathcal{Y},  \forall \rv N_i \in \mathrm{Dec}(\rv X, y), \ \rv Z \perp \rv N_i  \  \ \}$
\end{restatable}
\begin{proof}
Because of \cref{lemma:zeroVminimal} we have $\forall y \in \mathcal{Y}, \forall \rv N \in \decxy{}$ we have $\DIF{N}{Z_y}=0$.
As $\universal{}$-information recovers MI that means $\rv N \perp \rv Z_y$. So $\Usmin{} = \{ \rv Z \in \Usuff{} | \ \forall y \in \mathcal{Y},  \forall \rv N_i \in \mathrm{Dec}(\rv X, y), \ \rv Z \perp \rv N_i  \  \ \}$ as desired.
\end{proof}



\begin{restatable}[Monotonicity of $\V$-information]{lemma}{monotonicity}\label{lemma:monotonicity}
Let $\V,\mathfam{G} \subseteq \mathcal{P}(\mathcal{Y}|\mathcal{Z})$ 
be two predictive families such that $\V \subseteq \mathfam{G}$, then $\forall \rv Z$ t.v.i $\mathcal{Z}$ and $\forall \rv Y$ t.v.i. $\mathcal{Y}$ we have $\op{I_{\mathcal{G}}}{\rv Z \rightarrow \rv Y} \leq \DIF{Y}{Z}$.
\end{restatable}

\begin{proof}
Let us start from the monotonicity of the predictive entropy \cite{xu2020theory}, which comes directly from the fact that we are optimizing over a larger functional family:
\begin{align*}
\op{H_{\mathcal{G}}}{\rv Y | \rv Z} &\geq \op{H_{\mathcal{G}}}{\rv Y | \rv Z} & \text{Monotonicity $\V$-ent.} \\
\op{H}{\rv Y } - \op{H_{\mathcal{G}}}{\rv Y | \rv Z} &\leq \op{H}{\rv Y } - \op{H_{\mathcal{G}}}{\rv Y | \rv Z} \\
\op{I_{\mathcal{G}}}{\rv Z \rightarrow \rv Y} &\leq \DIF{Y}{Z} & \text{\cref{prop:marginalent}}
\end{align*}
\end{proof}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Optimality of $\V$-Minimality}
\label{appx:proof_optimal}

We will now prove the main result of our paper, namely that any ERM that uses a $\V$-minimal $\V$-sufficient representation will reach the best achievable test loss. 
The main difference with \cref{prop:opt_qsuf} is that the following talks about the optimality of \textit{any} ERMs rather than the existence of at least one such ERM.
Although the proof is relatively long, the intuition is quite simple. Here is a rough outline:

\begin{enumerate}
\item As the theorem is about \textit{all} ERMs, use a proof by contrapositive to only talk about a single ERM $\hat{f}^*$ that performs optimally on train but not on test.
\item Construct a random variable $\tilde{\rv N}$ which labels train examples as 1 and test as 0. Show that $ \tilde{\rv N} \in \decxy{}$
\item Due to the piecewise universality assumption, show that as $\hat{f}^* \in \V$ can distinguish between train and test then there is a $\tilde{f} \in \V$ that can predict $\tilde{\rv N}$ better than random. 
\item Show that it entails $\op{I_{\V}}{\rv Z \to \tilde{\rv N}} \neq 0$. Conclude by \cref{lemma:zeroVminimal} that $\rv Z \not \in \Qsmin{}$ as desired. 
\end{enumerate}


Formally:

\begin{theorem*}\label{theo:opt_qmin_formal} 
Let $\sampleD{}$ be a sampled dataset.
$\rv Z \in \Qsmin{}$  $\implies$  $\forall \hat{f}^* \in \hat{V}^*(\mathcal{D}, \rv Z)$ we have $(\hat{f}^*, \rv Z) \in (\V^*, \rv Z^*)$.
\end{theorem*}

\begin{proof}
For ease of notation we assume that we are in a binary classification setting $|\mathcal{Y}|=2$.
The proof generalizes to the multi-classification setting as well due to the invariance of $\V$ to label permutations.

We will prove the statement by contrapositive, namely $\exists \hat{f}^* \in \hat{V}^*(\mathcal{D}, \rv Z)$ s.t. $(\hat{f}^*, \rv Z) \not \in (\V^*, \rv Z^*)$   $\implies$   $\rv Z \not \in \Qsmin{}$.

The left hand side means that $\exists y \in \mathcal{Y}$ s.t. $\qCH{\hat{f}^*}{Y=y}{Z} \neq \eqCH{\hat{f}^*}{Y=y}{Z}{D} = 0 $.
Due to the deterministic labeling hypothesis and the $\V$-sufficiency of $\rv Z$ (\cref{lemma:VsuffSupp}), we can study one single such label $y$ without considering any other label $y'$ (neither the examples nor the representations interact between labels).

Let $\mathcal{X}^{t}_y$ be the set of examples (associated with $y$) seen during training and  $\mathcal{X}^{e}_y = \mathcal{X}_y \setminus \mathcal{X}^{t}_y$ those only during test (eval). 
Let $\mathcal{Z}^{w}_y \defeq \{ z_y \in \mathcal{Z}_y | \hat{f}^*[z_y](y) \neq 1 \}$ be the set of representation (associated with $y$) who are (wrongly) not given a probability of 1 for the correct label. 
Let $\mathcal{Z}^{c}_y \defeq \mathcal{Z}_y \setminus \mathcal{Z}^{w}_y $ be the set of representations that are (correctly) labeled $y$ by $\hat{f}^*$ with a probability of 1.

Let $\tilde{\rv N} \defeq  \mathds{1}[\rv X_y \in \mathcal{X}^t_y ]$.
I.e. a binary ``selector'' of training examples.
Note that $\tilde{\rv N} \in \decxy{}$, as $\mathds{1}[\cdot \in \mathcal{X}^t_y]$ is a deterministic function from $\mathcal{X}_y \to \mathcal{Y}$.
We will now show that $\op{I}{\rv Z_y \rightarrow \tilde{\rv N} }  \neq 0$.
I.e. $\op{H_{\mathcal{V}}}{\tilde{\rv N} \cond \rv Z_y} < \op{H}{\tilde{\rv N}}$.

\iffalse
First, let us derive $\op{H}{\rv N}$:
\begin{align*}
 - \op{H}{\rv N} 
 &\defeq P_{\tilde{\rv N}}(1) \log  P_{\tilde{\rv N}}(1) + P_{\tilde{\rv N}}(0) \log  P_{\tilde{\rv N}}(0) \\ 
 &=  \sum_{x_y \in \mathcal{X}_y} P_{\tilde{\rv N}, \rv X_y }(1, x_y) \log  P_{\tilde{\rv N}}(1) + 
 \sum_{x_y \in \mathcal{X}_y} P_{\tilde{\rv N}, \rv X_y }(0, x_y) \log  P_{\tilde{\rv N}}(0) \\ 
 &= \sum_{x_y \in \mathcal{X}_y^t} P_{\rv X_y }(x_y) \log  P_{\tilde{\rv N}}(1) + 
 \sum_{x_y \in \mathcal{X}_y^e} P_{\rv X_y }(x_y) \log  P_{\tilde{\rv N}}(0) & \text{Def. } \tilde{\rv N} \\ 
&= \sum_{x_y \in \mathcal{X}_y^t} \sum_{z_y \in \mathcal{Z}_y} P_{\rv X_y, \rv Z_y }(x_y, z_y) \log  P_{\tilde{\rv N}}(1) + 
 \sum_{x_y \in \mathcal{X}_y^e} 
 \sum_{z_y \in \mathcal{Z}_y}
 P_{\rv X_y, \rv Z_y  }(x_y, z_y) \log  P_{\tilde{\rv N}}(0) \\
&= \sum_{x_y \in \mathcal{X}_y^t} \sum_{z_y \in \mathcal{Z}_y^c} P_{\rv X_y, \rv Z_y }(x_y, z_y) \log  P_{\tilde{\rv N}}(1) + 
 \sum_{x_y \in \mathcal{X}_y^e} 
 \sum_{z_y \in \mathcal{Z}_y}
 P_{\rv X_y, \rv Z_y  }(x_y, z_y) \log  P_{\tilde{\rv N}}(0) & \text{ERM} \\
&= \sum_{x_y \in \mathcal{X}_y^t} \sum_{z_y \in \mathcal{Z}_y^c} P_{\rv X_y, \rv Z_y }(x_y, z_y) \log  P_{\tilde{\rv N}}(1)  + 
 \sum_{x_y \in \mathcal{X}_y^e} 
 \sum_{z_y \in \mathcal{Z}_y^c}
 P_{\rv X_y, \rv Z_y  }(x_y, z_y) \log  P_{\tilde{\rv N}}(0) \\
&+ 
 \sum_{x_y \in \mathcal{X}_y^e} 
 \sum_{z_y \in \mathcal{Z}_y^w}
 P_{\rv X_y, \rv Z_y  }(x_y, z_y) \log  P_{\tilde{\rv N}}(0) 
\end{align*}
Where the second to last line comes from the fact that $\hat{f}^*$ is an ERM, so all training examples were given the correct label with probability one to get an empirical risk of zero (\cref{lemma:existperfect}).
\fi

Let us now derive $\op{H_{\mathcal{V}}}{\rv N | \rv Z_y}$. 
Note that due to the piecewise universality assumption, we know that there exists a function $f_{P_{\rv Y}} \in V$ s.t. $\forall z_y \in \mathcal{Z}_y^c$ we have $f_{P_{\rv Y}}[z_y]=P_{\rv Y}$.

Let us denote by $f_c \in V$
\begin{align*}
 - \op{H_{\mathcal{V}}}{\rv N | \rv Z_y } 
 &\defeq 
 \sup_{f \in \V} \biggl(
 \sum_{z_y \in \mathcal{Z}_y}  P_{\tilde{\rv N}, \rv Z_y}(1, z_y) \log  f[z_y](1) \\
 &+ \sum_{z_y \in \mathcal{Z}_y}  P_{\tilde{\rv N}, \rv Z_y}(0, z_y) \log  f[z_y](0) 
 \biggr) \\
 &\geq   
 \sum_{z_y \in \mathcal{Z}_y}  P_{\tilde{\rv N}, \rv Z_y}(1, z_y) \log  f_c[z_y](1) \\
 &+ \sum_{z_y \in \mathcal{Z}_y}  P_{\tilde{\rv N}, \rv Z_y}(0, z_y) \log  f_c[z_y](0) 
  \\
 &= 
 \sum_{z_y \in \mathcal{Z}_y} \sum_{x_y \in \mathcal{X}_y}  P_{\tilde{\rv N}, \rv Z_y,\rv X_y}(1, z_y, x_y) \log  f_c[z_y](1) \\
 &+ \sum_{z_y \in \mathcal{Z}_y} \sum_{x_y \in \mathcal{X}_y}  P_{\tilde{\rv N}, \rv Z_y, \rv X_y}(0, z_y, x_y) \log  f_c[z_y](0) 
  \\
&=  
 \sum_{z_y \in \mathcal{Z}_y} \sum_{x_y \in \mathcal{X}_y^t}  P_{\rv Z_y,\rv X_y}(z_y, x_y) \log  f_c[z_y](1) \\
 &+ \sum_{z_y \in \mathcal{Z}_y} \sum_{x_y \in \mathcal{X}_y^e}  P_{\rv Z_y, \rv X_y}(z_y, x_y) \log  f_c[z_y](0) & \text{Def. }  \tilde{\rv N} 
  \\
&=  
 \sum_{z_y \in \mathcal{Z}_y^c} \sum_{x_y \in \mathcal{X}_y^t}  P_{\rv Z_y,\rv X_y}(z_y, x_y) \log  f_c[z_y](1)  & \text{Def. }  \hat{f}^*,f_c,\mathcal{Z}_y^c  \\
 &+ \sum_{z_y \in \mathcal{Z}_y^c} \sum_{x_y \in \mathcal{X}_y^e}  P_{\rv Z_y, \rv X_y}(z_y, x_y) \log  f_c[z_y](0)   \\
 &+ \sum_{z_y \in \mathcal{Z}_y^w} \sum_{x_y \in \mathcal{X}_y^e}  P_{\rv Z_y, \rv X_y}(z_y, x_y) \log  f_c[z_y](0) \\
 &=  
 \sum_{z_y \in \mathcal{Z}_y^c} \sum_{x_y \in \mathcal{X}_y^t}  P_{\rv Z_y,\rv X_y}(z_y, x_y) \log  P_{\rv X_t | \rv Z_y}( \rv X_t \in \mathcal{X}_y^t | \rv Z_y \in  \mathcal{Z}_y^c) & \text{Set } f_c  \\
 &+ \sum_{z_y \in \mathcal{Z}_y^w} \sum_{x_y \in \mathcal{X}_y^e}  P_{\rv Z_y, \rv X_y}(z_y, x_y) \log 
1 & \text{Set } f_c \\
&= - \op{H}{\tilde{\rv N} \cond \rv Z_y \in  \mathcal{Z}_y^c} & \text{Def. } \tilde{\rv N}\\
&> - \op{H}{\tilde{\rv N} \cond \rv Z_y} & \mathcal{Z}_y^c \neq \varnothing \\
&\geq  - \op{H}{\tilde{\rv N}} & \text{Conditioning} 
\end{align*}

We conclude that $\op{I}{\rv Z_y \rightarrow \tilde{\rv N} }  \neq 0$, so by \cref{lemma:zeroVminimal}, $\rv Z \not \in \Qsmin{}$ which concludes the proof.
\end{proof}

%{\color{red} to do : show that piecewise universality holds for NN with step wise activation}


\subsubsection{$\V$-Minimality $\V$-Sufficiency Properties}
\label{appx:proof_prop}


\Vminsuff*



\begin{proof}$ $
\begin{description}
\item[Monotonicty] From \cref{lemma:zeroVminimal} we know that $\V$-minimal $\V$-sufficient representation satisfy $\forall y \in \mathcal{Y}, \forall \rv N \in \decxy{}$ we have $\DIF{N}{Z_y}=0$.
Following the same steps, we can show that the same holds when both functional family (with respect to which one is minimal and sufficient) are different.
As a result, we know that $\forall y \in \mathcal{Y}, \forall \rv N \in \decxy{}$  : $\op{I_\mathcal{G}}{\rv Z_y \rightarrow \rv N}=0$.
Using the monotonocity of $\V$-information in our setting (\cref{lemma:monotonicity}) we have $0 = \op{I_{\mathcal{G}}}{\rv Z_y \rightarrow \rv N}  \leq  \DIF{N}{Z_y} $.
As $\V$-information is always positive, we conclude that $\forall y \in \mathcal{Y}, \forall \rv N \in \decxy{}$,  $\DIF{N}{Z_y}=0$.
By \cref{lemma:zeroVminimal}, we conclude that $\rv Z$ is $\V$-minimal $\V$-sufficient as desired.
%
\item[Characterization]
As $\DIFxzCy{}$ is an average over a non negative (positivity of $\V$information) $\DIF{N}{Z_y}$ it is equal to zero if and only if all the terms are zero.
Now let $\rv Z \in \Qsuff{}$ be $\V$-sufficient then $\rv Z \in \Qsuff{} \DIFxzCy{} = 0  \iff \rv Z \in \Qsuff{} \forall y \in \mathcal{Y}, \forall \rv N \in \decxy{} \iff \forall \rv Z \in \Qsmin{}$ where the last $\iff$ comes from \cref{lemma:zeroVminimal}.
This concludes the proof.
%
\item[Recoverability]
Using \cref{prop:recsuff} we know that $\Usuff{}=\suff{} \cap \mathcal{Z}$ so the domain of optimization for minimality and $\universal{}$-minimality is the same.
Using \cref{prop:charminsuff} and \cref{prop:charUminUsuff} we only need to show that both characterizations are the same. I.e. $\forall \rv Z \in \Usuff{}$ we have $\rv Z \perp \rv X | \rv Y \iff \rv N_i \perp \rv Z_y, \ \forall \rv N_i \in \mathrm{Dec}(\rv X, y), \forall y \in \mathcal{Y}$.
As a reminder for the following, $\rv Z_y$ and $\rv X_y$  have by definition distribution $P_{\rv X_y} \defeq P_{\rv X | y}$,$P_{\rv Z_y} \defeq P_{\rv Z | y}$. 

($\implies$) Starting from minimality $\rv Z \perp \rv X | \rv Y $ so $\forall y \in \mathcal{Y}$ we have $P_{\rv X_y, \rv Z_y}=P_{\rv X, \rv Z |y}=P_{\rv X | y}*P_{\rv Z |y}=P_{\rv X_y}*P_{\rv Z_y}$ from which we conclude that $\rv Z_y \perp \rv X_y$.
As,  $\rv N_i = t'_i( \rv X_y)$ we also have $\rv Z_y \perp \rv N_i$, $\forall \rv N_i \in \decxy{}$ as desired.\\

($\impliedby$) Let us prove it by contrapositive. I.e. we show that $\rv Z \not \perp \rv X | \rv Y \implies \exists y \in \mathcal{Y}, \exists \rv N_i \in \mathrm{Dec}(\rv X, y) \ s.t. \  \rv N_i \not\perp \rv Z_y $.
As $\rv Z \not \perp \rv X | \rv Y$ then  $\exists \Tilde{x} \in \mathcal{X}, \Tilde{y} \in \mathcal{Y}$ s.t. $P_{\rv Z |\rv X, \rv Y } (\cdot \cond \Tilde{x},\Tilde{y})  \neq P_{\rv Z| \rv Y}(\cdot \cond \Tilde{y})$.
Let us define  $ \tilde{\rv N} = \mathds{1}[\rv X_{\tilde{y}}  = \tilde{x}_{\tilde{y}}] $,
as $\mathds{1}[\rv X_{\tilde{y}}  = \cdot ]$ is a deterministic function from $\mathcal{X}_{\tilde{y}} \to \mathcal{Y}$, we have $\tilde{\rv N} \in \mathrm{Dec}(\rv X, \tilde{y})$.
Then:
\begin{align*}
P_{\rv Z_\tilde{y}| \tilde{\rv N}}(\cdot \cond 1) 
&= P_{\rv Z| \tilde{\rv N}, \rv Y}(\cdot \cond 1, \tilde{y}) & \text{Def. } \rv Z_\tilde{y} \\
&= P_{\rv Z |\rv X, \rv Y } (\cdot \cond \Tilde{x},\Tilde{y}) & \text{Def. }  \tilde{\rv N} \\
&\neq P_{\rv Z| \rv Y}(\cdot \cond \Tilde{y}) & \text{Def. }  \tilde{x},\tilde{y} \\
&= P_{\rv Z_{\tilde{y}}} & \text{Def. }  \rv Z_{\tilde{y}}
\end{align*}
As $P_{\rv Z_{\tilde{y}} | \tilde{\rv N}}(\cdot \cond 1)  \neq P_{\rv Z_{\tilde{y}}}$ we conclude that $\exists \tilde{y} \in \mathcal{Y}, \exists \rv N_i \in \mathrm{Dec}(\rv X, \tilde{y}) \ s.t. \  \rv N_i \not\perp \rv Z_{\tilde{y}} $ as desired.
\end{description}
\end{proof}

\yann{to do corrolary optimality of min suff}






==> appendices/proof_old.tex <==
\section{Theoretical Results and Proofs}

\ydnote{The following has to be a rearranged / cleaned / clarified. I'm currently making sure the proof are correct rather than clear.
}

\subsection{Background}
\label{sec:proof_bckgrnd}

A standard and more detailed review of information theory and probabilistic supervised learning can be found in \citet{cover2012elements} and \citet{gressmann2018probabilistic} respectively.


\begin{restatable}[Strict Properness of Log Loss]{proposition}{properness}\label{prop:proper}
\ydnote{Should remove and simply cite: there's nothigng non standard here}
$\forall x \in \mathcal{X}$ and $\forall Q_{\hrv Y \cond \rv x} \in [\mathcal{X} \to \mathcal{P}(\mathcal{Y})]$ not equal to $P_{\rv Y \cond \rv x}$:
\[\E{y \sim P_{\rv Y \cond \rv x}}{S(y,P_{\rv Y \cond x})} < \E{y \sim P_{\rv Y \cond \rv x}}{S(y,Q_{\hrv Y \cond x})}\]
%We say that the log loss $S$ is a strictly proper scoring rule.
\end{restatable}

%\properness*
\begin{proof}
For notational convenience we use the respective probability mass functions $p,q$ of $P_{\rv Y \cond \rv z=z},Q_{\hrv Y \cond \rv Z=z}$. 

\begin{align*}
\Delta &\defeq 
\E{y \sim P_{\rv Y \cond \rv z=z}}{S(y,Q_{\hrv Y \cond \rv Z=z})} - \E{y \sim P_{\rv Y \cond \rv z=z}}{S(y,P_{\rv Y \cond \rv Z=z})} \\
&= -\sum_{y \in \mathcal{Y}} p(y \cond z) \log q(y \cond z) - \sum_{y \in \mathcal{Y}} -p(y \cond z) \log p(y \cond z) \\
&= \sum_{y \in \mathcal{Y}} p(y \cond z) \log \frac{p(y \cond z)}{q(y \cond z)} & \text{$p,q$ same support}\\
&= \KL{P_{\rv Y \cond \rv z=z},Q_{\hrv Y \cond \rv Z=z}} \\ 
&> 0 & \text{$p \neq q$}
\end{align*}
Where the last line comes from the positive definiteness of the KL divergence when $p \neq q$.
\end{proof}

\begin{restatable}[Data Processing Inequality]{proposition}{dpi}\label{prop:dpi}
If $\rv Y - \rv X - \rv Z$ is a Markov Chain then $ \op{H}{\rv Y \cond \rv Z} \geq \op{H}{\rv Y \cond \rv x}$.
\end{restatable}

%\dpi*
\begin{proof}
By substracting $\op{H}{\rv Y}$ on both sides from the standard DPI \cite{cover2012elements}.
\end{proof}

\begin{restatable}[Invariance to Bijections]{proposition}{bij}\label{prop:bij}
If $f$ is a bijection then $\op{H}{\rv Y} = \op{H}{f(\rv Y)}$ .
\end{restatable}

\begin{proof}
(intuition) change of discrete variable with bijection \ydnote{check : http://www.stat.umn.edu/geyer/f11/5101/notes/n1.pdf, https://www.math.arizona.edu/~jwatkins/f-transform.pdf, https://www.randomservices.org/random/dist/Transformations.html, http://www.math.umd.edu/~millson/teaching/STAT400/slides/article9.pdf}. 
\end{proof}

\begin{corollary}\label{cor:bij}
If $f$ is a bijection then $\op{H}{\rv Z \cond \rv X} = \op{H}{f(\rv Z) \cond \rv X}$ and $\op{H}{\rv X \cond \rv Z} = \op{H}{\rv X \cond  f(\rv Z)}$.
\end{corollary}

\begin{proof}
Letting $\rv Y = (\rv Z, \rv X)$ in \cref{prop:bij} we have $\op{H}{\rv Z,\rv X} = \op{H}{f(\rv Z ,\rv X)}$ for any bijection. Let $g$ also be a bijection, then $f(\cdot)=(g(\cdot),\cdot)$ is a bijection and we thus have $\op{H}{\rv Z,\rv X} = \op{H}{g(\rv Z),\rv X}$ substracting $\op{H}{\rv X}$ both sides we get $\op{H}{\rv Z \cond  \rv X} = \op{H}{g(\rv Z) \cond \rv X)}$. By the same argument with a bijection $g'$ and letting $f(\cdot)=(\cdot,g'(\cdot))$ we get $\op{H}{\rv X \cond  \rv Z} = \op{H}{g'(\rv X) \cond \rv Z}$ which concludes the proof.
\end{proof}

Note that the previous proposition and corollary only hold because of our simplifying assumption of finite sample spaces. 
In the case of continuous r.v., it is nevertheless possible to show that if $f$ is a homeomorphism (i.e. smooth bijection) then $\op{H}{\rv X \cond \rv Z} = \op{H}{\rv X \cond  f(\rv Z)}$. This can be proven by the invariance of mutual information to homeomorphisms \cite{kraskov2004estimating}.
So the intuition that we give in the main text of conditional entropy not being the right measure for the quality of a representation still holds for continuous r.v. as one could entangle representations in a very non linear fashion without affecting conditional entropy.

In the following, we will prove the equivalence between our definition of (minimal) sufficient statistics and the standard ones.
Note that in the main text we allow ourselves to work with stochastic representations. 
This contrasts with the definition of statistic, namely that a statistic $\rv Z$ of $\rv X$ is any composition between a measurable function $E$ and $\rv X$ (essentially deterministic representations).
As standard minimality and sufficiency is not defined for ``stochastic statistics'', we only show the equivalence for deterministic statistics.
\ydnote{Here I only prove the equivalence with predictive sufficient statistics which recovers the usual sufficient statistics if $\rv Y = \Theta$ \tocite{}}

\begin{definition}[Standard Sufficient Statistic]\label{def:standard_sufficiency}
A statistic $\rv Z$ of $\rv X$ is said predictive sufficient for $\rv Y $ if $\rv Y - \rv Z - \rv X$ forms a Markov Chain.
\end{definition}

\begin{proposition}[Equivalence of Sufficient Statistics]
Let $\rv Y, \rv X$ be two random variables, and $E$ a deterministic function.
A statistic $\rv Z \defeq E(\rv X)$ of $\rv X$ is predictive sufficient for $\rv Y$ by \cref{def:standard_sufficiency} if and only if it is sufficient for $\rv Y$ by \cref{def:predictive_min}.
\end{proposition}

\begin{proof}
First, assume that $\rv Z$ is sufficient by \cref{def:standard_sufficiency}. Namely, $\rv Y - \rv X - \rv Z$ constitutes a Markov Chain.
From the data processing inequality (DPI) we have $\MI{Y}{X} \geq \MI{Y}{Z}$. Since $\rv Z$ is sufficient, we also have $\rv Y - \rv Z - \rv X $. Using again the DPI, we have $\MI{Y}{Z} \geq  \MI{Y}{X}$. Due to the upper and lower bound we must have $\MI{Y}{X} = \MI{Y}{Z}$. This can be further decomposed as $\op{H}{\rv Y} - \op{H}{\rv Y \cond \rv X} = \op{H}{\rv Y} - \op{\rv H}{\rv Y \cond \rv Z}$, from which we conclude that $\op{H}{\rv Y \cond \rv X} = \op{H}{\rv Y \cond \rv Z}$.

For the second direction, assume that $\rv Z$ is sufficient by \cref{def:predictive_min}. 
 Using the chain rule of information we have 
 \begin{align*}
\MI{Y}{Z,\rv X} &= \MI{Y}{Z ,\rv X}\\
\MI{Y}{Z}+\MI{Y}{X \cond \rv Z}&=\MI{Y}{X}+\MI{Y}{Z \cond \rv X}\\
\op{H}{\rv Y} - \op{H}{\rv Y \cond \rv Z} +\MI{Y}{X \cond \rv Z} &= \op{H}{\rv Y}- \op{H}{\rv Y \cond \rv X} +\MI{Y}{Z \cond \rv X}\\
- \op{H}{\rv Y \cond \rv Z} +\MI{Y}{X \cond \rv Z} &=- \op{H}{\rv Y \cond \rv X} +\MI{Y}{Z \cond \rv X}\\
- \op{H}{\rv Y \cond \rv Z} +\MI{Y}{X \cond \rv z}&=- \op{H}{\rv Y \cond \rv Z} +\MI{Y}{Z \cond \rv X} & \text{\cref{def:predictive_min}}\\
\MI{Y}{X \cond \rv z}&= \MI{Y}{z \cond \rv X} \\
\MI{Y}{X \cond \rv z}&= 0 & \rv Y - \rv X - \rv Z \\
 \end{align*}
 
 Where the last line used the fact that $\rv Z$ is a statistic of $\rv X$.  
 $\MI{Y}{X \cond Z}= 0$, implies that $\rv Y - \rv Z - \rv x$ is a Markov chain, which concludes the proof.
\end{proof}

\begin{definition}[Standard Minimal Sufficient Statistic]\label{def:standard_minimality}
A sufficient statistic $\rv Z$ of $\rv X$ for $\rv Y$ is said \textit{minimal} if for any other sufficient statistic $\rv Z'$ of $\rv X$ for $\rv Y$, there exists a measurable function $g$ such that $\rv Z = g(\rv Z')$ almost everywhere.
\end{definition}

\begin{proposition}[Equivalence of Sufficient Statistics]
Let $\rv Z$ denote a \textit{sufficient} statistic of $\rv X$ for $\rv Y$.
Then it is called minimal by  \cref{def:standard_minimality} if and only if it is minimal by \cref{def:predictive_min}.
\end{proposition}

\begin{proof}
 Let $\rv Z$ be minimal by \cref{def:standard_minimality}, then $\forall \rv Z' \in \suff{}$ we have  the Markov Chain $\rv X - \rv Z' - \rv Z $. 
 From the DPI, $\op{H}{\rv X} - \op{H}{\rv X \cond \rv Z} = \MI{X}{Z} \leq \MI{ X}{Z'} = \op{H}{\rv X} - \op{H}{\rv X \cond \rv Z'}$. Rearranging we have $\op{H}{\rv X \cond \rv Z} \geq \op{H}{\rv X \cond \rv Z'}$. This completes the first direction of the proof.
 
For the other direction, suppose $\rv Z \defeq E(\rv X)$ is not minimal by \cref{def:standard_minimality}, i.e. there exists a sufficient statistic $\rv Z' \defeq E'(\rv X)$ such that there is no function $g$ that satisfies $f(\rv X) = g(E'(\rv X))$. 
Then the binary relation $\{(E'(x), E(x)) \cond x \in \mathcal{X}\}$ is not univalent, therefore the converse relation $\{(E(x),E'(x)) \cond x \in \mathcal{X}\}$ is not injective.
As a result, there exists a non injective function $\Tilde{g}$ such that
$E'(\rv X) = \Tilde{g}(E(\rv X))$. 
From the DPI we have $\op{H}{\rv X} - \op{H}{\rv X \cond \rv Z'} = \MI{X}{Z'} < \MI{ X}{Z} = \op{H}{\rv X} - \op{H}{\rv X \cond \rv Z}$ with a strict inequality due to the non injectivity of $\Tilde{g}$.
In summary, we supposed $\rv Z$ was not minimal by \cref{def:standard_minimality} and found that $\op{H}{\rv X \cond \rv Z} < \op{H}{\rv X \cond \rv Z'}$ meaning that $\rv Z$ is not minimal by \cref{def:predictive_min}.
By contrapositive, we conclude that minimality by \cref{def:predictive_min} implies minimality by \cref{def:standard_minimality}, thus concluding the proof.
\end{proof}



\subsection{Conditional Entropy}
\label{sec:proof_dif}

%FOr reasons 

%In this section we will discuss why the decodable entropy is defined as it is and what are the properties it satisfies.
%Conditional entropy is a well studied operator that has many desirable properties \tocite{} and is fundamental for information theory (as mutual information can be decomposed in an entropy and conditional entropy term). 
%We strongly believe that it is useful but have argued in the main text that it is is not completely satisfactory as it does not take into account the functional family at hand.
%The main issue is that it is defined using the underlying conditional distribution, which might not be available in a given constrained functional family.
%Due to the strict properness of the log loss \tocite{} we know7 that the underlying conditional distribution is optimal, and as a result would like the notion of decodable entropy to recover conditional entropy when it is not constrained. 
%We will call this property \textbf{weak recoverability}

%\begin{lemma}\label{lem:bij}
%$\op{H}{\rv X \cond \rv Z} = \op{H}{\rv Y \cond \rv Z} \forall \rv Z$ if and only if there exists a bijection $f$ s.t. $\rv X = f(\rv Y)$.
%\end{lemma}
%\begin{proof}
%(intuition) if a bijection exists then $\op{H}{\rv X \cond \rv Z} = \op{H}{\rv Y \cond \rv Z} \forall %\rv Z$ because of the discrete change of variable with a bijection \ydnote{check : http://www.stat.umn.edu/geyer/f11/5101/notes/n1.pdf, https://www.math.arizona.edu/~jwatkins/f-transform.pdf, https://www.randomservices.org/random/dist/Transformations.html, http://www.math.umd.edu/~millson/teaching/STAT400/slides/article9.pdf}.

%(intuition) For the second direction, suppose $\op{H}{\rv X \cond \rv Z} = \op{H}{\rv Y \cond \rv Z} \forall \rv Z$ then we also have that it is true for $\rv Z = \rv Y$ in other words $\op{H}{\rv X \cond \rv Y}=\op{H}{\rv Y \cond \rv Y}=0$ meaning that there exists a function $f$ s.t. $\rv X = f(\rv Y)$. 
%Using the same argument for $\rv Z = \rv X$, we get that $\op{H}{\rv Y \cond \rv X}=\op{H}{\rv X \cond \rv X}=0$ so there exists a function $f^{-1}$ s.t. $\rv Y = f^{-1}(\rv X)$. Putting both equations together we have $\rv Y = f^{-1}(f(\rv Y))$ so $f$ is a bijection.
%\end{proof}


\begin{definition}[Decomposition of Random Variables]\label{def:decomp}
A collection of r.v. $\rv N=\{\rv N_i\}_i$ is a $\mathcal{Y}$ decomposition of a on constant $\rv X$.
If 
\begin{itemize}
\item \textbf{Take value in $\mathcal{Y}$}. Each $\rv N_i \in \rv N$ t.v.i in a set $\mathcal{N}$ whose support is a subset of $\mathcal{Y}$ : $\mathrm{supp}(\mathcal{N}) \subseteq \mathcal{Y}$. 
\item \textbf{Bijection} There exists a bijection $f$ s.t. $\rv X = f(\rv N)$;
\item \textbf{Independence} $\rv N_i \perp \rv N_j, \ \forall \rv N_i \in \rv N \neq \rv N_j \in \rv N$.
\item \textbf{Not Constant} There are no constant r.v. $\rv N_i$.
\end{itemize}
\end{definition}

\begin{restatable}[General Decodable Entropy]{definition}{gen_decentropy}\label{def:gen_q_entropy}
The decodable entropy of $\rv X$ (regardless of its sample space $\mathcal{X}$) conditioned on $\rv Z$ with respect to $\family{} \in [\mathcal{Z} \to \mathcal{P}(\mathcal{Y})]$, is:
\[
\CHF{X}{z} 
\defeq \E{\rv N \sim \mathrm{dec}_{\mathcal{Y}}(\mathcal{X})}{\sum_{N_i \in \rv N}\CHF{N_i}{Z}}
\]
Where $\mathrm{dec}_{\mathcal{Y}}(\rv X)$ is the set of all $\mathcal{Y}$ decompositions of $\mathcal{X}$.
\end{restatable}

In the main body, we gave a slightly different definition which is equivalent but more computationally efficient to work with in the considered task. It uses the base $\mathcal{Y}$ expansion of $\rv X$ instead of the $\mathcal{Y}$ decompositions of $\rv X$.

\expansion*

\begin{restatable}[Decodable Entropy]{definition}{decentropy}\label{def:q_entropy}
The decodable entropy \footnote{A more general definition that encompasses any $\rv X$ under a single equation is discussed in \cref{sec:proof_dif}. Although more general it is slightly more difficult to understand and not useful for our setting. Indeed, in machine learning one always samples a dataset from a distribution, so the empiricial random variable can always be rewritten as a uniform random variable over indices of the dataset.} of $\cdot$ conditioned on $\rv Z$ with respect to $\family{} \in [\mathcal{Z} \to \mathcal{P}(\mathcal{Y})]$, is:
\begin{itemize}
\item \textbf{Simple Case} if $\cdot=\rv Y$ t.v.i $\mathcal{Y}$
\[
\CHF{y}{z} 
\defeq 
\inf_{Q \in \mathfam{Q}} \E{n_i,z \sim P_{\rv N_i \times \rv z}}{S(n_i,\pred{}))} 
\]
\item \textbf{Complex Case} if $\cdot=\rv X$ t.v.i. $\mathcal{X} \neq \mathcal{Y}$ and with distribution $P_{\rv X}=\mathrm{Unif}(\mathcal{X})$. Let $(\rv N_i)_i$ be a base $|\mathcal{Y}|$ expansion of $\rv X$ then 
\[
\CHF{X}{z} 
\defeq \sum_{i=0}^{\ceil{\log_{|\mathcal{Y}|}(|\mathcal{X}|)}-1} \CHF{N_i}{Z}
\]
\end{itemize}
%Where $\rv N_i$ is the $i^{th}$ coefficient of the base $|\mathcal{Y}|$ expansion of a predefined $\mathrm{ind}(x)$. \ydnote{This is not well explained, but I don't know how to do it a more clear fashion. Hopefully the previous paragraph makes it clear though.}
\end{restatable}

Importantly, both definitions are equivalent for the considered cases as we will now show.

\begin{lemma}\label{lem:expansion_decomposition}
Let $|\mathcal{Y}|=[0,\dots,|\mathcal{Y}|-1]$, then any base $|\mathcal{Y}|$ expansion of a $\mathcal{X}$ with uniform distribution $P_{\rv X}=\mathrm{Unif}(\mathcal{X})$ is also a $\mathcal{Y}$ decomposition of $\rv X$.
\end{lemma}
\begin{proof}
\item \textbf{Take value in $\mathcal{Y}$}. Let $\rv N = (\rv N_i)_i$ be a base $|\mathcal{Y}|$ expansion of $\mathcal{X}$, then by definition  $\forall \rv N_i$ there exists $f_i : \mathcal{X} \to [0, \dots ,|\mathcal{Y}|-1]$ s.t. $\rv N_i = f_i(\rv X)$. Due to our multi-class classification assumption, $\mathcal{Y}=[0, \dots ,|\mathcal{Y}|-1]$ from which we conclude that $\rv N_i$ t.v.i $\mathcal{Y}$.
\item \textbf{Bijection}  Let $f^{-1} : \mathcal{Y}^{\ceil{\log_b{\mathcal{X}}}-1} \to [0, \dot ,|\mathcal{X}|-1]$ a function that maps $\rv N \mapsto \sum_{i=0}^{\ceil{\log_b{\mathcal{X}}}-1} \rv N_i b^{i}$.
Applying it to the base $|\mathcal{Y}|$ expansion of $\mathcal{X}$ :  $\rv N = (\rv f_i(\rv X))_i$ we get $\forall x \in \mathcal{X}$:
\begin{align*}
f^{-1}((\rv f_i(x))_i) 
&= \sum_{i=0}^{\ceil{\log_b{\mathcal{X}}}-1} f_i(x) b^{i} \\
&= \mathrm{ind}(x)  \\
\mathrm{ind}^{-1}f^{-1}((\rv f_i(x))_i)  &= x & \text{Def. Property}  \\
\end{align*}
Where the last line comes from the defining property of a $|\mathcal{Y}|$ expansion of $\mathcal{X}$ which ensures that $\mathrm{ind}$ is a bijection, and thus invertible as both sides of the equality are defined on $[0, \dot ,|\mathcal{X}|-1]$. Putting all together we get that $g=\mathrm{ind}^{-1}f^{-1}$ is a bijection and $\rv X = g(\rv N)$.
\item \textbf{Independence} .
\item \textbf{Not Constant} .
\end{proof}


\begin{proposition}
\cref{def:q_entropy} is equivalent to \cref{def:gen_q_entropy} for the two cases that are considered.
\end{proposition}
\begin{proof} 
\hfill
\begin{itemize}
\item \textbf{Simple Case} Let $\rv Y$ t.v.i $\mathcal{Y}$ and $\CHF{y}{z}$ be as defined in \cref{def:gen_q_entropy}, then :
\begin{align*}
\CHF{X}{z} 
&\defeq \E{\rv N \sim \mathrm{dec}_{\mathcal{Y}}(\rv X)}{\sum_{N_i \in \rv N}\CHF{N_i}{Z}} \\
&= \E{\rv N \sim \mathrm{dec}_{\mathcal{Y}}(\rv X)}{\CHF{N_0}{Z}} & \text{Singleton $\rv N$} \\
&= \E{f \sim \{f' \in [\mathcal{Y} \to \mathcal{Y}] \ s.t. \ f' \text{is a bijection} \} }{\op{H}{f(\rv N_0),\rv Z}} & \text{Bijection} \\
&= \CHF{Y}{Z} & \text{Inv. to Perm.} \\
\end{align*}
Where the second line used the fact that the number of $\rv N_i \in \rv N$ has to be $m=1$. 
Indeed, by the definition of a $\mathcal{Y}$ decomposition of $\rv Y$ there needs to be a bijection between $\rv N$ and $\rv Y$ meaning that the cardinality of their respective sample space has to be equal. 
The cardinality the sample space of $\rv N$ is $|\mathcal{N}|=|\mathcal{Y}|^m$  --- each $\rv N_i$ is non constant and t.v.i $\mathcal{Y}$ --- so $m=1$ to satisfy $|\mathcal{N}|=|\mathcal{Y}|^m=|\mathcal{Y}|$.
The third line used the fact that if $m=1$ then the set of all decompositions $\mathrm{dec}_{\mathcal{Y}}(\rv Y) = \{f(\rv Y) \ s.t. \ f \text{vis a permutation of } \rv Y \}$, where a permutation is a bijection where the domain and codomain coincide.
The last line used the invariance of the predictive family $\family{}$ to permutations.
%%%
\item \textbf{Complex Case} Let $\rv X$ t.v.i. $\rv X$ t.v.i. $\mathcal{X} \neq \mathcal{Y}$ with distribution $P_{\rv X}=\mathrm{Unif}(\mathcal{X})$ and $\CHF{x}{z}$ be as defined in \cref{def:gen_q_entropy}, then :
\begin{align*}
\CHF{X}{z} 
&\defeq \E{\rv N \sim \mathrm{dec}_{\mathcal{Y}}(\rv X)}{\sum_{N_i \in \rv N}\CHF{N_i}{Z}} \\
&= \E{\rv N \sim \mathrm{dec}_{\mathcal{Y}}(\rv X)}{\CHF{N_0}{Z}} & \text{Singleton $\rv N$} \\
&= \E{f \sim \{f' \in [\mathcal{Y} \to \mathcal{Y}] \ s.t. \ f' \text{is a bijection} \} }{\op{H}{f(\rv N_0),\rv Z}} & \text{Bijection} \\
&= \CHF{Y}{Z} & \text{Inv. to Perm.} \\
\end{align*}
Where the f
\end{itemize}
\end{proof}










\begin{lemma}[Decomposition and Weak Recoverability]\label{lem:weak}
Let $\rv N = ( \rv N_i )_i$ be a random vector with component $\rv N_i$ then $\sum_{\rv N_i \in \rv N } \inf_{U \in \mathfam{U}} \E{n_i,z \sim P_{\rv N_i \times \rv z}}{S(n_i,U_{\hrv N_i \cond z}))} = \op{H}{\rv X \cond \rv Z }$ $\forall \rv Z$ if and only if $\rv N$ is a $\mathcal{Y}$ decomposition of $\rv X$.
\end{lemma}

\begin{proof}
\begin{description}
\item[Take value in $\mathcal{Y}$] Suppose $\exists i \ s.t. \ \rv N_i$ does not satisfy the $\mathcal{Y}$-requirement. Then there exists $n_i \not\in \mathcal{Y}$, which happens with non zero probability. As a result, $S(n_i,U_{\hrv N_i \cond z}))=- \log(U_{\hrv N_i \cond z}(n_i \cond z))$ is not well defined (because the codomain of $U_{\hrv N_i \cond z}$ is wrong) . The expectation over $\rv N_i$ is thus also not well defined (as $U$ t.v.i in $\mathcal{P}(\mathcal{Y})$ ).
\item[Bijection and Independence] 
First let us show that if $\rv N$ is a $\mathcal{Y}$ decomposition of $\rv X$ , then $\sum_{\rv N_i \in \rv N } \inf_{U \in \mathfam{U}} \E{n_i,z \sim P_{\rv N_i \times \rv z}}{S(n_i,U_{\hrv N_i \cond z}))} = \op{H}{\rv X \cond \rv Z }$:
\begin{align*}
\op{\Tilde{H}_{\mathfam{U}}}{\rv X \cond \rv Z} &= \sum_{\rv N_i \in \rv N } \inf_{U \in \mathfam{U}} \E{n_i,z \sim P_{\rv N_i \times \rv z}}{S(n_i,U_{\hrv N_i \cond z}))} \\
&= \sum_{\rv N_i \in \rv N } \E{n_i,z \sim P_{\rv N_i \times \rv z}}{S(n_i,P_{\hrv N_i \cond  z}(n_i \cond z)} & \text{Strictly Proper} \\
&= \sum_{\rv N_i \in \rv N } \op{H}{\rv N_i \cond \rv Z} & \text{Definition} \\
&= \op{H}{(\rv N_i)_i \cond \rv Z} & \text{Independence} \\
&= \op{H}{f((\rv N_i)_i) \cond \rv Z} & \text{\cref{cor:bij}} \\
&= \op{H}{\rv X \cond \rv Z} 
\end{align*}
Where the second line uses the strict properness of the log loss and the fact that $P_{N_i \cond \rv z} \in [\mathcal{Z} \to \mathcal{P}(\mathcal{Y})] \eqdef \universal{}$. 
Where the last line comes from the assumption that there exists a bijection $f$ s.t. $\rv X = f(\rv N)$.
This proves the first direction. 

For the other direction , suppose that $\sum_{\rv N_i \in \rv N } \inf_{U \in \mathfam{U}} \E{n_i,z \sim P_{\rv N_i \times \rv z}}{S(n_i,U_{\hrv N_i \cond z}))} = \op{H}{\rv X \cond \rv Z }$ $\forall \rv Z$.
Using the strict properness of the log loss (as before) we get that $\sum_{\rv N_i \in \rv N } \op{H}{\rv N_i \cond \rv Z} = \op{H}{\rv X \cond \rv Z}, \ \forall Z$.

Set $\rv Z = \rv X$ then $\sum_{\rv N_i \in \rv N } \op{H}{\rv N_i \cond \rv X} = \op{H}{\rv X \cond \rv X} = 0$. 
As conditional entropy is non-negative (discrete case), then we must have $\op{H}{\rv N_i \cond \rv X}=0, \ \forall i$. From which we conclude that $\forall i$ there exists $f_i$ s.t. $\rv N_i = f_i(\rv Z)$.
Similarly set $\rv Z = \rv N$ then $\op{H}{\rv N_i \cond \rv N}=0, \ \forall N_i \in \rv N$ so $\op{H}{\rv X \cond \rv N } = \sum_{\rv N_i \in \rv N } \op{H}{\rv N_i \cond \rv X} = 0$ from which we conclude that there is a function $f^{-1}$ s.t. $\rv X = f^{-1}(\rv N)$. 
Putting it with the previous equation we have $\rv X = f^{-1}(\rv N) = f^{-1}((\rv N_i)_i) =  f^{-1}(( f_i(\rv X) )_i)$ from which we conclude that $f(\cdot)=(f_i(\cdot))_i$ is a bijection.

Finally, suppose $\rv Z$ is independent of $\rv X$. As there exists a bijection between $\rv N$ and $\rv X$ we also have that $\rv Z \perp \rv N$ so
\begin{align*}
\op{H}{\rv X } 
&= \op{H}{\rv X \cond \rv Z} & \rv Z \perp \rv X \\
&= \sum_{\rv N_i \in \rv N } \op{H}{\rv N_i \cond \rv Z} & \text{Supposition} \\
&= \sum_{\rv N_i  } \op{H}{\rv N_i} & \rv Z \perp \rv N \\
&\geq \op{H}{(\rv N_i)_i }  \\
&= \op{H}{f((\rv N_i)_i)} & \text{\cref{cor:bij}} \\
&= \op{H}{\rv X } 
\end{align*}
Obviously $\op{H}{\rv X } = \op{H}{\rv X} $ so the inequality has to be an equality $\sum_{\rv N_i } \op{H}{\rv N_i} = \op{H}{(\rv N_i)_i }$. I.e. $\rv N_i \perp \rv N_j, \forall i \neq j$, which concludes the proof.
\end{description}
\end{proof}

It has the following desirable properties

\propentropy*
\begin{proof}
\begin{description}
%\item[Positivity] The log score is non-negative  $S(n_i,\pred{}) = - \log Q(n_i|\rv Z) \geq 0$ and expectations, infimums, and sums preserve non-negativity. Note that this only holds because discreteness assumptions of r.v (finite sample spaces). 
%\item[Independence] By the independence property of conditional entropy $\op{H}{\cdot \cond \rv z} = \op{H}{\cdot}$ if and only if $\cdot \indep \rv z$.
\item[Monotonicity] Let $\family{} \subseteq \pFam{\mathfam{G}}$, $\mathcal{A}_i \defeq \{\E{n_i ,z \sim P_{\rv N_i \times \rv z}}{S(n_i,\pred{}))} \ s.t. \ \pred{} \in \family{} \}$, and $\mathcal{B}_i \defeq \ \{\E{n_i,z \sim P_{\rv N_i \times \rv Y}}{S(n_i,\pred{}))} \ s.t. \ \pred{} \in \pFam{\mathfam{G}} \}$.
The image of a subset under a mapping is the subset of the image, so we have $\mathcal{A}_i \subseteq \mathcal{B}_i$.
By the subset property of infimums $\mathcal{A}_i \subseteq \mathcal{B}_i$ implies $\inf \mathcal{A}_i \geq \inf \mathcal{B}_i$, $\forall i = 0, \dots, \ceil{\log_{|\mathcal{Y}|}(|\mathcal{X}|)}-1$.
As the previous inequality holds for all $i$, we have that the inequality also holds for the sum of all terms : $\CHF{X}{Z} = \sum_{0}^{\ceil{\log_{|\mathcal{Y}|}(|\mathcal{X}|)}-1} \inf \mathcal{A}_i \geq \sum_{0}^{\ceil{\log_{|\mathcal{Y}|}(|\mathcal{X}|)}-1} \inf  \mathcal{B}_i = \op{H_{\mathfam{G}}}{\rv X, \rv Z}$. 
\item[Weak Recoverability] We want to show $\op{H}{\rv X \cond \rv z} =  \op{H_{\mathfam{U}}}{\rv X \cond \rv z} \defeq \sum_{i=0}^{\ceil{\log_{|\mathcal{Y}|}(|\mathcal{X}|)}-1} \inf_{U \in \mathfam{U}} \E{n_i,z \sim P_{\rv N_i \times \rv z}}{S(n_i,U_{\hrv N_i \cond z}))}$. Given the form of the last equation, we can apply \cref{lem:weak}, which stipulates that the weak recoverability property is satisfied if and only if $(\rv N_i)_i$ is a $\mathcal{Y}$ decomposition of $\mathcal{X}$.
By definition $(\rv N_i)_i$ is a base $|\mathcal{Y}|$ expansion of $\rv X$, so we just need to show that it implies 
\item[Strong Recoverability]
Note that from the strict properness of the log loss, $\forall \rv Z$ and $\forall \hat{Q}_{\rv Y \cond \rv z} \neq P_{\rv Y \cond \rv z}$, we have:
\begin{align}
\E{y \sim P_{\rv Y \cond \rv z}}{S(y,P_{\rv Y \cond z})} &< \E{y \sim P_{\rv Y \cond \rv z}}{S(y,Q_{\hrv Y \cond z})} \nonumber \\
 \op{H}{\rv Y \cond \rv z} \defeq \E{y,z \sim P_{\rv Y \rv z}}{S(y,P_{\rv Y \cond z})} &< \E{y,z \sim P_{\rv Y \rv z}}{S(y,Q_{\hrv Y \cond z})} \label{eqn:expected_proper}  
\end{align}
For the first direction of the proof, suppose that $P_{\rv Y \cond \rv Z} \in \family{}$ but $\op{H}{\rv Y \cond \rv z} \neq \CHF{y}{z}$. 
Then either $\op{H}{\rv Y \cond \rv z} > \CHF{y}{z}$ or $\op{H}{\rv Y \cond \rv z} < \CHF{y}{z}$.
The former contradicts 
For the second part of the proof, we have to use our assumptions of finite sample sets $\mathcal{Z}$
This comes directly from the properness of log loss (\cref{prop:proper}).
$P_{\rv Y \cond \rv Z} \in \family{}$ if and only if $\op{H}{\rv Y \cond \rv X} =  \CHF{y}{x}$. 
\end{description}


\textbf{Recoverability}: \yann{NOT FINISHED !}
Note that from the strict properness of the log loss, $\forall \rv Z$ and $\forall \hat{Q}_{\rv Y \cond \rv z} \neq P_{\rv Y \cond \rv z}$, we have:
\begin{align}
\E{y \sim P_{\rv Y \cond \rv z}}{S(y,P_{\rv Y \cond z})} &< \E{y \sim P_{\rv Y \cond \rv z}}{S(y,Q_{\hrv Y \cond z})} \nonumber \\
 \op{H}{\rv Y \cond \rv z} \defeq \E{y,z \sim P_{\rv Y \rv z}}{S(y,P_{\rv Y \cond z})} &< \E{y,z \sim P_{\rv Y \rv z}}{S(y,Q_{\hrv Y \cond z})} \label{eqn:expected_proper}  
\end{align}

For the first direction of the proof, suppose that $P_{\rv Y \cond \rv Z} \in \family{}$ but $\op{H}{\rv Y \cond \rv z} \neq \CHF{y}{z}$. 
Then either $\op{H}{\rv Y \cond \rv z} > \CHF{y}{z}$ or $\op{H}{\rv Y \cond \rv z} < \CHF{y}{z}$.
The former contradicts 

For the second part of the proof, we have to use our assumptions of finite sample sets $\mathcal{Z}$

This comes directly from the properness of log loss (\cref{prop:proper}).
$P_{\rv Y \cond \rv Z} \in \family{}$ if and only if $\op{H}{\rv Y \cond \rv X} =  \CHF{y}{x}$. 

\end{proof}


In this section we will show that 

Intuitively, the decomposition should be such that
\begin{inlinelist}
\item $\rv N_i$ t.v.i $\mathcal{Y}$ thus having a well defined $\CHF{N_i}{Z}$;
\item the collection $\rv N$ has all (and only) the information in $\rv X$;
%I.e. we want $\op{H}{\rv X} = \op{H}{\rv N_1, \dots, \rv N_n} = \op{I}{\rv X;\rv N_1, \dots, \rv N_n}$.
\item all $\rv N_i$ should ``carry'' different information about $\rv X$, thus keeping $|\rv N|$ small and avoiding unnecessary computation.
%I.e. all $N_i$ should be independent of each other.
\end{inlinelist}


The exact requirements for the decomposition to be valid are formalized in the following definitions.

\begin{definition}[Decomposition of Random Variables]
A collection of r.v. $\rv N=\{\rv N_i\}_i$ is a $\mathcal{Y}$ decomposition of $\rv X$.
If 
\begin{inlinelist}
\item $\forall \rv N_i \in \rv N, \ \exists $ a function $f_i : \mathcal{X} \to \mathcal{Y}$ s.t. $\rv N_i = f_i(\rv X)$;
\item $\exists f^{-1}$ s.t. $\rv X = f^{-1}(\rv N)$;
\item $\rv N_i \perp \rv N_j, \ \forall \rv N_i \in \rv N \neq \rv N_j \in \rv N$.
\end{inlinelist}
\ydnote{Maybe a little dense in math symbols. I can use more space, use more English word, but I think that the previous paragraph does most of the job on the intuition. Although the definition is important to understand the definition of $\CHF{N_i}{Z}$ it is not crucial to understand in practice as we will only use a very specific decomposition (the minimal one). }
\end{definition}

The smallest set of 


$\family{} \subseteq \pFam{\mathfam{G}}$ then $\CHF{y}{z} \geq \op{H_\mathfam{G}}{\rv Y \cond \rv z}$ 

\propDI*
\begin{proof}
\yann{\textbf{Recoverability} : Already proved recoverablity for predictive entropy, so has to only do it for uninformative. If the underlying marginal is in the proper predictive family, this means that $\exists z$ s.t. $Q_{\rv Y \cond z}=P(\rv Y)$. In other words the marginal is in the range of the family. By definition of a predictive family it means that there's a predictor that will output the marginal regardless of the input. As log loss is proper scoring, this is the best achievable => inf.
\textbf{Independence} : If Independence then by definition, product of marginals is equal to joint => get 0 as the predictive entropy becomes the uninformative one. 
\textbf{Non negativity} :  Unconditional is weighted average (expectation over x) of conditional cross entropy, so to minimize it will chose a predictor which constantly predicts the minimal cross entropy. Because the family is proper, the informed predictive entropy could also predict the same marginal => at least as good.
}
\end{proof}

\subsection{Learning Optimal Representations}

%\sufficiencies*
\begin{proof}
\yann{Last equality comes directly from the definition. First inclusion is trivially true if $\mathcal{S}_{\mathcal{Q}}$ is empty. If it is not empty, it comes from the fact that any $Q_{\rv Y \cond \rv Z=z}$ would by definition be $P_{\rv Y \cond \rv X=x}$. This will usually only be a subset as any ``any bijection applied to Z which cannot be inverted by Q would be sufficient but not Q-sufficient''. Second inclusion comes from the fact that $\mathcal{G} \subseteq \mathcal{U}$.}
\end{proof}


\qminimallink*
\proof{
\begin{itemize}
\item \textbf{Rademacher Complexity}
First let us prove that any $\family{}$-sufficient statistic, which yields the minimum Rademacher complexity is a minimal $\family{}$-sufficient statistic. 
\end{itemize}
}

%%%%%%%%%%%%%%%%
\subsection{$\mathcal{Q}$-Decodable Information Bottleneck}



\optimalqib*

\begin{proof}\label{proof:qib}
\yann{HAS TO BE UPDATED FOR THE NEW DEFINITION + GENERALIZED }

First, let us assume that we have access to an oracle that gave us $q(\rv Y \cond \rv Z)$ and $q'(\rv Y \cond \varnothing)$ as defined in \cref{eqn:q_yz}. 
Important variational derivatives are \footnote{For simplicity, we will use the following abuse of notation $\int_{ Z} z p(z) \defeq \int  Z(w) P(\sd{w})$.
Note that we are integrating over the underlying measure, such that the derivation holds for any distributions (continuous or not).}:

\begin{align*} 
%%%%%%%%%
\partial_{\rv z \to \rv y} 
&\defeq
\frac{\partial}{\partial p(z \cond x) } \op{DI_{\mathcal{Q}}}{ Z \to  Y}
\nonumber  \\
%
&= \frac{\partial}{\partial p(z \cond x) } \int_{ Z',  Y} p(z' \cond y)p(y) \log \frac{q(y \cond z')}{q(y \cond \varnothing)} \nonumber \\
%
&= \int_{ Z',  Y} p(x \cond  y) \delta_z(z') p(y) \log \frac{q(y \cond z')}{q(y \cond \varnothing)} \nonumber \\
%
&= \int_{Y} p(x \cond y)p(y) \log \frac{q(y \cond z')}{q(y \cond \varnothing)} \nonumber \\
%
&= p(x) \int_{ Y} p(y \cond x) \log \frac{q( y \cond z)}{p(y)} \frac{q(y \cond z')}{q(y \cond \varnothing)} \nonumber  \\
%
&= - p(x) \biggl( \KL{p( Y \cond x), q(Y \cond z)} \nonumber  \\
& - \KL{p( Y \cond x), p(Y)} 
 \biggr) 
\end{align*}

\begin{align*}
%%%%%%%%%
\partial_{\rv z , \rv x} &\defeq 
\frac{\partial}{\partial p(z \cond x) } \op{I}{ X;  Z} \\
&= \frac{\partial}{\partial p(z \cond x) } \int_{ Z',  X'} p(z' \cond x')p(x') \log \frac{p(z' \cond x')}{p(z')} \nonumber \\
%
&= \int_{ Z',  X'} \delta_z( z')\delta_x( x') p(x') \log \frac{p(z' \cond x')}{p(z')} \nonumber \\
&+ \int_{ Z',  X'} p(x') \frac{p(z')\delta_x(x') - p(x)}{p(z' \cond x')p(z')} \delta_z( z')
\nonumber \\
%
&=  p(x) \log \frac{p(z \cond x)}{p(z)}  
+ \int_{ X'} p(x')  \delta_x(x') \\
&- \int_{ X'} p(x' \cond z) p(x) 
\nonumber \\
%
&=  p(x) \br{\log \frac{p(z \cond  x)}{p(z)}  + 1 - 1}
\nonumber \\
%
&=  p(x) \log \frac{p(z \cond x)}{p(z)}
\end{align*}

We can now minimize the Lagrangian [eqn]:

\begin{align*} 
0 &= \frac{\partial}{\partial p(z \cond x) } \op{\mathcal{L}}{p( Z \cond  X)} \nonumber \\
%
&= \partial_{\rv z , \rv x} - \beta \partial_{\rv z \to \rv y} 
\\
%
&= p(x) \biggl( \log \frac{p(z \cond x)}{p(z)}  + \beta \KL{p( Y \cond x), q(Y \cond z)}  \\
& - \beta \KL{p( Y \cond x), q(Y \cond \varnothing)} \biggr) \\
%
\log p(z \cond x) &= \log p(z) - \beta \KL{p( Y \cond x), q(Y \cond z)} \\
&+ \beta \KL{p( Y \cond x), q(Y \cond \varnothing)}  \\
%
 p(z \cond x) &= \frac{p(z)}{C(Y,x,\beta)}\exp \pa{- \beta \KL{p( Y \cond x), q(Y \cond z)}} 
\end{align*}

With $C(Y,x,\beta) = \exp \pa{- \beta \KL{p( Y \cond x), q(Y \cond \varnothing)}}$

Let us now replace $q(\rv Y \cond \rv Z)$ and $q'(\rv Y \cond \varnothing)$ with their definitions.
Note that $q(\rv Y \cond \rv Z)$ depends itself on $p(z \cond x) $, which is why we needed to use an oracle that provides us with the optimal $q(\rv Y \cond \rv Z)$ \textit{conditioned} on the optimal $p(z \cond x)$ which we are looking for.

%We assumed that every function $q \in \mathcal{Q}$ outputs a valid distribution over $\mathcal{Z}$.
%A very similar derivation can be done in the more general case by constraining $\int_{ Z} p(z \cond  x) = 1 \ \forall x \in \mathcal{X}$, which would add $\int_{ X} \lambda(x) \br{\int_{ Z} p(z \cond  x) - 1 }$ to the Lagrangian.
%This term would not change [eqn], as it would result in adding $\lambda(x)$ in the exponent of $C(\rv Y, x, \beta)$.
\end{proof}

\blahut*


\begin{proof}
For the main parts of the proof, we refer the reader to the same theorem with vanilla information bottleneck \cite{tishby2000information}.
Here, we only prove that the theorem still holds with our changes, namely when replacing $\KL{p( Y \cond x), p(Y \cond z)}$ with $\KL{p( Y \cond x), q(Y \cond z)}$ and adding the [last self consitent eqn].

First, note that the parts of \cite{tishby2000information} proofs that depend on $\KL{p( Y \cond x), p(Y \cond z)}$ only uses the positivity of the term. 
This still holds when replacing $p(Y \cond \rv z)$ with $q(Y \cond \rv z)$.

Now, to prove convergence, we have to show that the Lagrangian [eqn] decreases at every [last self consitent eqn].

\begin{align*}
\CHF{Y}{X}^{t+1} &<  \CHF{Y}{X}^{t} \\
\op{H_\mathcal{Q}}{Y} - \CHF{Y}{X}^{t+1} &> \op{H_\mathcal{Q}}{Y} - \CHF{Y}{X}^{t} \\
\DIF{Z}{Y}^{t+1} &> \DIF{Z}{Y}^{t} \\
-\beta \DIF{Z}{Y}^{t+1} &< -\beta \DIF{Z}{Y}^{t} \\
\MI{Z}{X} -\beta \DIF{Z}{Y}^{t+1} &< \MI{Z}{X} -\beta \DIF{z}{Y}^{t} \\
\op{\mathcal{L}}{q^{t+1}(Y \cond \rv z)} &< \op{\mathcal{L}}{q^{t}(Y \cond \rv z)} 
\end{align*}

Where we have used the fact that $\MI{Z}{X}$ and $\op{H_\mathcal{Q}}{Y}$ are independent of  $q(Y \cond \rv z)$.

\end{proof}

Importantly from a practical perspective, the last self-consistent equation just requires  $q^{t+1}(Y \cond z)$ to be ``better'' than the previous one (if it can). 
It does not require to chose the best possible $q$ in the functional class $\mathcal{Q}$ which would usually be computationally infeasible.

It is also important to note that the Blahut-Arimoto algorithm was 
\begin{inlinelist}
\item Convex in the vanilla rate distortion setting; 
\item Conditionally convex (but not jointly) in the information bottleneck setting;
\item Not conditionally convex in the DIB (due to last self-consistent equation) but still convergent.
\end{inlinelist}

==> appendices/proofs_dif.tex <==

\subsection{Conditional Information}
\label{sec:proof_dif}

\textbf{decentropy}

It has the following desirable properties
\textbf{propentropy}

\begin{proof}
\begin{description}
\item[Monotonicity] Essentially because the infimum is taken over a larger set.
Let $\family{} \subseteq \pFam{\mathfam{G}}$, $\mathcal{A}_i \defeq \{\E{n_i ,z \sim P_{\rv N_i \times \rv z}}{L(n_i,\pred{}))} \ s.t. \ \pred{} \in \family{} \}$, and $\mathcal{B}_i \defeq \ \{\E{n_i,z \sim P_{\rv N_i \times \rv Y}}{S(n_i,\pred{}))} \ s.t. \ \pred{} \in \pFam{\mathfam{G}} \}$.
The image of a subset under a mapping is the subset of the image, so we have $\mathcal{A}_i \subseteq \mathcal{B}_i$.
By the subset property of infimums $\mathcal{A}_i \subseteq \mathcal{B}_i$ implies $\inf \mathcal{A}_i \geq \inf \mathcal{B}_i$, $\forall \rv N_i \in \rv N $.
As the previous inequality holds for all $\rv N_i$, we have that the inequality also holds for the sum of all terms : $\CHF{X}{Z} = \sum_{\rv N_i \in \rv N} \inf \mathcal{A}_i \geq \sum_{\rv N_i \in \rv N} \inf  \mathcal{B}_i = \op{H_{\mathfam{G}}}{\rv X, \rv Z}$. 
Conclude because $\op{H}{Y}$ is a constant. 
%
\item[Non negativity] First show it $\DIF{N_i}{Z}$. Because of our assumption on the predictive family we know that there exists a predictor that always predicts using the marginal. Because of the infimum $H_Q[Y|Z]$ can only be smaller than that, so $H[Y]-H_Q[Y|Z]$ has to be greater than 0.
Sum of non negative terms is non negative terms so we have $\DIF{X}{Z}$ because each $\DIF{N_i}{Z}$ are non negative (as just shown).
%
\item[Independence] 
First we show it for $\DIF{N_i}{Z}$
\begin{align}
\CHF{N_i}{Z} &= \inf_{Q \in Q} \E{n_i ,z \sim P_{\rv N_i \times \rv z}}{- \log q(n_i|z)))}    & \text{definition} \\
&= \inf_{Q \in Q}\E{n_i \sim P_{\rv N_i}}{ \E{z \sim P_{\rv z}}{- \log q(n_i|z)))}}   & \text{independence} \\
&\geq \E{n_i \sim P_{\rv N_i}}{- log \E{z \sim P_{\rv z}}{ q(n_i|z)))}}   & \text{jensen} \\
&= \inf_{Q \in Q} \E{n_i \sim P_{\rv N_i}}{- log q(n_i)))}   & \text{marginalize} \\
&= \op{H}{\rv N_i} &{Strict properness} \\
\end{align}
Where the last line uses the strict properness of the log loss (so the best marginal predict is the underlying marginal) and the fact that we assumed that there is a predictor that always predicts with the true marginal in $\mathfam{Q}$.
We thus have $\op{H}{\rv N_i} - \CHF{N_i}{Z} \leq 0 $ but we know that positive (proved above) so $\DIF{N_i}{Z}=0$.
Let's tackle $\DIF{X}{Z}$, we know that if $\rv X \perp \rv Z$ then $\MI{X}{Z}=0$. As MI is invariant to bijections and $\rv N_i$ are independent we have $0=\MI{X}{Z}=\MI{\{\rv N_i\}_i}{Z}=\sum_{\rv N_i}=\MI{N_i}{Z}$ from which we conclude that each $\rv N_i$ is independence of $\rv Z$. 
We can thus apply our previous proof on each component $\DIF{X}{Z}=\sum_{\rv N_i} \DIF{N_i}{Z}=0$.
\end{description}
\end{proof}

Let's now prove that we generalize MI and $\mathcal{V}$ information.


\begin{lemma}[Decomposition and Recoverability of Conditional Entropy]\label{lem:weak}
Let $\rv N = ( \rv N_i )_i$ be a random vector with component $\rv N_i$ then $\sum_{\rv N_i \in \rv N } \inf_{U \in \mathfam{U}} \E{n_i,z \sim P_{\rv N_i \times \rv z}}{S(n_i,U_{\hrv N_i \cond z}))} = \op{H}{\rv X \cond \rv Z }$ $\forall \rv Z$ if and only if $\rv N$ is a $\mathcal{Y}$ decomposition of $\rv X$.
\end{lemma}

\begin{proof}
\begin{description}
\item[Take value in $\mathcal{Y}$] Suppose $\exists i \ s.t. \ \rv N_i$ does not satisfy the $\mathcal{Y}$-requirement. Then there exists $n_i \not\in \mathcal{Y}$, which happens with non zero probability. As a result, $S(n_i,U_{\hrv N_i \cond z}))=- \log(U_{\hrv N_i \cond z}(n_i \cond z))$ is not well defined (because the codomain of $U_{\hrv N_i \cond z}$ is wrong) . The expectation over $\rv N_i$ is thus also not well defined (as $U$ t.v.i in $\mathcal{P}(\mathcal{Y})$ ).
\item[Bijection and Independence] 
First let us show that if $\rv N$ is a $\mathcal{Y}$ decomposition of $\rv X$ , then $\sum_{\rv N_i \in \rv N } \inf_{U \in \mathfam{U}} \E{n_i,z \sim P_{\rv N_i \times \rv z}}{S(n_i,U_{\hrv N_i \cond z}))} = \op{H}{\rv X \cond \rv Z }$:
\begin{align*}
\op{\Tilde{H}_{\mathfam{U}}}{\rv X \cond \rv Z} &= \sum_{\rv N_i \in \rv N } \inf_{U \in \mathfam{U}} \E{n_i,z \sim P_{\rv N_i \times \rv z}}{S(n_i,U_{\hrv N_i \cond z}))} \\
&= \sum_{\rv N_i \in \rv N } \E{n_i,z \sim P_{\rv N_i \times \rv z}}{S(n_i,P_{\hrv N_i \cond  z}(n_i \cond z)} & \text{Strictly Proper} \\
&= \sum_{\rv N_i \in \rv N } \op{H}{\rv N_i \cond \rv Z} & \text{Definition} \\
&= \op{H}{(\rv N_i)_i \cond \rv Z} & \text{Independence} \\
&= \op{H}{f((\rv N_i)_i) \cond \rv Z} & \text{bijection req.} \\
&= \op{H}{\rv X \cond \rv Z} 
\end{align*}
Where the second line uses the strict properness of the log loss and the fact that $P_{N_i \cond \rv z} \in \PYZ = \universal{}$. 
Where the last line comes from the assumption that there exists a bijection $f$ s.t. $\rv X = f(\rv N)$.
This proves the first direction. 

For the other direction , suppose that $\sum_{\rv N_i \in \rv N } \inf_{U \in \mathfam{U}} \E{n_i,z \sim P_{\rv N_i \times \rv z}}{S(n_i,U_{\hrv N_i \cond z}))} = \op{H}{\rv X \cond \rv Z }$ $\forall \rv Z$.
Using the strict properness of the log loss (as before) we get that $\sum_{\rv N_i \in \rv N } \op{H}{\rv N_i \cond \rv Z} = \op{H}{\rv X \cond \rv Z}, \ \forall Z$.

Set $\rv Z = \rv X$ then $\sum_{\rv N_i \in \rv N } \op{H}{\rv N_i \cond \rv X} = \op{H}{\rv X \cond \rv X} = 0$. 
As conditional entropy is non-negative (discrete case), then we must have $\op{H}{\rv N_i \cond \rv X}=0, \ \forall i$. From which we conclude that $\forall i$ there exists $f_i$ s.t. $\rv N_i = f_i(\rv X)$.
Similarly set $\rv Z = \rv N$ then $\op{H}{\rv N_i \cond \rv N}=0, \ \forall N_i \in \rv N$ so $\op{H}{\rv X \cond \rv N } = \sum_{\rv N_i \in \rv N } \op{H}{\rv N_i \cond \rv N} = 0$ from which we conclude that there is a function $f^{-1}$ s.t. $\rv X = f^{-1}(\rv N)$. 
Putting it with the previous equation we have $\rv X = f^{-1}(\rv N) = f^{-1}((\rv N_i)_i) =  f^{-1}(( f_i(\rv X) )_i)$ from which we conclude that $f(\cdot)=(f_i(\cdot))_i$ is a bijection.

Finally, suppose $\rv Z$ is independent of $\rv X$. As there exists a bijection between $\rv N$ and $\rv X$ we also have that $\rv Z \perp \rv N$ so
\begin{align*}
\op{H}{\rv X } 
&= \op{H}{\rv X \cond \rv Z} & \rv Z \perp \rv X \\
&= \sum_{\rv N_i \in \rv N } \op{H}{\rv N_i \cond \rv Z} \\
&= \sum_{\rv N_i  } \op{H}{\rv N_i} & \rv Z \perp \rv N \\
&\geq \op{H}{(\rv N_i)_i }  \\
&= \op{H}{f((\rv N_i)_i)} & \text{\cref{cor:bij}} \\
&= \op{H}{\rv X } 
\end{align*}
Obviously $\op{H}{\rv X } = \op{H}{\rv X} $ so the inequality has to be an equality $\sum_{\rv N_i } \op{H}{\rv N_i} = \op{H}{(\rv N_i)_i }$. I.e. $\rv N_i \perp \rv N_j, \forall i \neq j$, which concludes the proof.
\end{description}
\end{proof}


\textbf{specialcase}

\begin{proof}
\begin{description}
\item[$\mathcal{V}$-information] The simplest $\mathcal{Y}$ decomposition of $\rv Y$ is $\rv N= \{\rv Y\}$. In this case there is only one element in the sum, and the definition the decodable information becomes the same as the $\mathcal{V}$-information. Any $\rv N= \{f(\rv Y)\}$ where $f$ is a bijection, would also be a valid $\mathcal{Y}$ decomposition, but that would not change the decodable entropy \ydnote{write in math all of that} because the predictive family is invariant to bijections on $\mathcal{Y}$.
We now have to show that with the assumptions made $\op{H}{\rv Y} = \op{H_\mathcal{V}}{\rv Y | \varnothing}$ \ydnote{shoudl rewrite their definition and optional ignorance !} . $\op{H_\mathcal{V}}{\rv Y | \varnothing}$ does not take into account the input, in which case \ydnote{write that formally} the best predictor is the underlying marginal (because of strict properness). Because of our assumption on the predictive family we can always predict using the underlying marginal so $\op{H}{\rv Y} = \op{H_\mathcal{V}}{\rv Y | \varnothing}$.
%
\item[Mutual Information] Given the form of the decodable entropy (link) equation, we can apply \cref{lem:weak}, and conclude that $\mathfam{U}$ decodable entropy recovers coditional entropy if and only if $(\rv N_i)_i$ is a $\mathcal{Y}$ decomposition of $\mathcal{X}$.
We thus have $\op{H}{X|Z}=\op{H_{\mathfam{U}}}{X|Z}$.
As $\{ \rv N_i\}$ is a decomposition of $\rv X$ we also have $\op{H}{\rv X}=\sum_{\rv N_i} \op{H}{\rv N_i}$.
Putting all together $\DI{\mathcal{U}}{X}{Z} = (\sum_{\rv N_i} \op{H}{\rv N_i}) - \op{H_{\mathfam{U}}}{X}{Z} = \op{H}{\rv X} - \op{H}{X|Z} = \MI{X}{Z}$.
\end{description}
\end{proof}





==> appendices/randlab.tex <==
\subsection{The Importance of Base $|\mathcal{Y}|$ Expansion Labeling}
\label{sec:appx_randlab}

\yann{Unreferenced}


\david{Rewrite if algorithm stays here}
\Cref{theo:opt_qmin} states that representations that maximize $\CHF{X}{Z}$ are optimal.
But the same holds [cite lemma] for representations that minimize the predictability of any random label.
In \cref{sec:theory_opt_rep} we argued that we are effectively minimizing the predictability of random labels [cite lemma] but propose a way to use only a specific set of possible labels of cardinality $\log_{|\mathcal{Y}|}(\mathcal{X})$ instead of all $|\mathcal{Y}|^{|\mathcal{X}|}$ possible random labels.
One interesting practical question is whether using these specific possible labels is better than randomly selecting the same number of possible labels from the entire set.
Indeed, although the former are optimal then latter might also be good  as [talk about the fact that typical sets have high entropy and low correlation => likely will cover].

\input{figures/algorithms/baseb}


\input{figures/randlab/randlab}

\Cref{fig:randlab} compares the effect of using [5,15,25,50,100] random labels instead of base expansions on Alice's log likelihood.
All other hyperparameters are identical to the ones used to generate \cref{fig:qmin_joint}.
For comparison, we also trained a DIB model which minimizes the base expansion for different indexing of $\mathcal{X}$.
Indeed, increasing the number of random labels might help as we do not have access to a global optimizer and each head will find different predictors due to their different initialization.
We see that ...




As discussed in \cref{sec:practical_optim}, the DIB formulation (like the IB formulation) gives rise to a trade-off between removing information about the input and preserving information about the label.
Such trade-off comes from Lagrangian relaxation.
To illustrate this, let's look at the IB objecive and its solution : minimal sufficient representations.
Due to the sufficient constraint we have $\op{H}{\rv Y \cond \rv Z }$ is a constant, meaning that maximizing $\op{H}{\rv X \cond \rv Z }$ cannot remove information about $\rv Y$ from $\rv Z$:

\begin{align*}
\smin{} &\defeq \arg \max_{Z \in \suff{}} \op{H}{\rv X \cond \rv Z } \\
&= \arg \max_{Z \in \suff{}} \op{H}{\rv X , \rv Y \cond \rv Z } & \rv Y - \rv X - \rv Z\\
&= \arg \max_{Z \in \suff{}} \op{H}{\rv X  \cond \rv Z , \rv Y}  + \op{H}{\rv Y \cond \rv Z }  & \text{Chain Rule} \\
&= \arg \max_{Z \in \suff{}} \op{H}{\rv X  \cond \rv Z , \rv Y}   + (Const)  & \text{Sufficiency} \\
&= \arg \max_{Z \in \suff{}} \op{H}{\rv X  \cond \rv Z , \rv Y}  
\end{align*}

We see that minimal representations can  be recovered by minimizing $\op{H}{\rv X  \cond \rv Z , \rv Y}$ instead of $\op{H}{\rv X  \cond \rv Z}$.
This can also be seen in the IB loss by incrementing $\beta$ by 1:

\begin{align*}
\mathcal{L}_{IB}^{\beta + 1}&= 
\op{I}{\rv X ; \rv Z} - (\beta+1) \op{I}{\rv y ; \rv Z} \\
&= 
\op{I}{\rv X, \rv Y ; \rv Z } - \op{I}{\rv y ; \rv Z} - \beta \op{I}{\rv y ; \rv Z} \\
&= 
\op{I}{\rv X ; \rv Z \cond \rv Y} + \op{I}{\rv y ; \rv Z} - \op{I}{\rv y ; \rv Z} - \beta \op{I}{\rv y ; \rv Z} \\ 
&= 
\op{I}{\rv X ; \rv Z \cond \rv Y}  - \beta \op{I}{\rv y ; \rv Z} \\ 
&= 
\mathcal{L}_{CIB}^{\beta }
\end{align*}

In theory, $\mathcal{L}_{CIB}^{\beta }$ is thus not very helpful as it is equivalent to $\mathcal{L}_{IB}$ with a different $\beta$.
In practice though, this might give rise to very different solutions as the estimation procedure can be different.
In the variational estimation case, this has been discussed in \cite{CIB}.

In our case we maximize  $\CHF{X}{Z}$ while minimizing $\CHF{Y}{Z}$ to make sure that no decodable information about $\rv Y$ is removed.
As we use an approximation procedures for optimization (no global optima), it is very probable that we end up removing a lot of information about $\rv Y$ when trying to remove information about $\rv X$.
To avoid this issue, we would also like to optimize $\op{H_{\V}}{\rv X   \cond  \rv Z}$ without changing $\op{H_{\V}}{\rv Y   \cond \rv Z}$.
We see two ways of doing it :

\begin{itemize}
\item $\Qsmin{} = \arg \max_{\rv z \in \Qsuff{}}\CHF{X}{Z} - \CHF{Y}{Z}$, which we will refer to as $\Delta$ DIB.
This might seem useless as it still requires estimating $\CHF{X}{Z}$. 
But (in some cases) we can actually directly estimate $\CHF{X}{Z} - \CHF{Y}{Z}$ without computing $\CHF{X}{Z}$.
Indeed, $\CHF{X}{Z} \defeq \sum_{\rv N_i \in \rv N} \CHF{N_i}{Z} $ so if we can set one of $\rv N_i$ to be equal to  $\rv Y$ then $\CHF{X}{Z} - \CHF{Y}{Z} = \sum_{\rv N_i \neq \rv Y} \CHF{N_i}{Z}$.
Practically this means that we need one less head and only need to remove predictability of indices in a given class (i.e. start indexing from 0 for every class).
The only problem with this, is that it is only exact if each $\rv N_i$ are independent (which is the case for balanced datasets).
\item $\Qsmin{} = \arg \max_{\rv z \in \Qsuff{}} \op{H_{\V}}{\rv X   \cond  \rv Z, \rv Y}$, which we will refer to as Conditional DIB.
This requires defining $\op{H_{\V}}{\rv X   \cond  \rv Z, \rv Y}$, which is not straightforward as $\V$ has $\mathcal{Z}$ as domain, not $\mathcal{Z}\times\mathcal{Y}$.
This can nevertheless be done exactly \ydnote{by exactly I mean that I keep the recoverability of $\op{H}{\rv X   \cond  \rv Z, \rv Y}$ } :
\begin{align*}
\op{H_{\V}}{\rv X   \cond  \rv Z, \rv Y} &\defeq \E{y \in P_{\rv Y}}{\op{H_{\V}}{\rv X   \cond  \rv Z, y}} \\
&= \E{y \in P_{\rv Y}}{\sum_{\rv N_i} \inf_{Q \in \V} \sum_n \sum_x \sum_z p(x,n \cond y) p(z \cond x, n, y) \log q(n \cond z, y))} \\
&= \E{y \in P_{\rv Y}}{\sum_{\rv N_i} \inf_{Q \in \V} \sum_n \sum_x \sum_z p(x,n \cond y) p(z \cond x) \log q(n \cond z))}
\end{align*}
The key is to realize that $q(n \cond z, y)=q(n \cond z)$ as the infimum is taken inside the expectation over $\rv Y$.
Practically speaking it means that for a given possible labeling $\rv N_i$ we do not need to use a single predictor but can use a different predictor for each class.
This is always possible, but suffers from the fact that it needs a number of predictors that is linear in $|\mathcal{Y}|$.
\end{itemize}

\input{figures/cdib/cdib}

We hypothesize that the Conditional and the $\Delta$ DIB objectives \ydnote{I will also look at the approximated CDIB by concatenating Y to Z. But probably won't put it in the paper, as it's hard to motivate theoretically (although practically will probably work well).} will be much more robust to varying $\beta$ than DIB and might even remove the need of hyperparamer tuning $\beta$ altogether. 
We compare both methods, and the non conditional version in \cref{fig:cdib} and see that ....



==> figures/Qmin2d/Qmin2d.tex <==
\begin{figure}
\centering
\subfloat[Emp. \vsufficient]{
\includegraphics[width=.47\textwidth]{figures/Qmin2d/databinmnist_run1_beta_modelcdib_reps_clfs.png}
  \label{fig:qmin2d_suff}
  }%
\subfloat[\vminimal and Emp. \vsufficient ]{
\includegraphics[width=.47\textwidth]{figures/Qmin2d/databinmnist_run1_beta_modelerm_reps_clfs.png}
\label{fig:qmin2d_min}
  }%
%\subfloat[Scaling Up]{
%  \includegraphics[width=.47\textwidth]{figures/Qsuf/QsufHeatmap.png}\label{fig:scaled_qsuf}}
\caption{Simple illustration of the role of \vminimality on worst-case generalization, encouraging indistinguishability for examples from the same class. Plots show the 2D representations encoded by an MLP on MNIST for binary classification (odd/even) as well as the decision boundary of a worst-case ERM in $\V$. Stars correspond to testing, circles to training. The model was trained on 200 examples.
In (a) the representation is trained to be empirically \vsufficient;
In (b) we add an additional \vminimality constraint.

}
\label{fig:qmin2d}
\end{figure}

==> figures/QminJoint/QminJoint.tex <==
\begin{figure}
\centering
\subfloat[Generalization Gap]{
\includegraphics[width=.47\textwidth]{figures/QminJoint/gap_loglike.png}
 \label{fig:qminjoint_gap_loglike}
  }%
\subfloat[Test Loglike.]{
\includegraphics[width=.47\textwidth]{figures/QminJoint/test_loglike.png}
 \label{fig:qminjoint_test_loglike}
  }%
 \hfill
\subfloat[$\CHF{Y}{Z}$]{
\includegraphics[width=.47\textwidth]{figures/QminJoint/train_H_Q_yCz_trnsf.png}
 \label{fig:qminjoint_train_H_Q_yCz}
  }%
 \subfloat[$\CHFbob{X}{Z}$]{
\includegraphics[width=.47\textwidth]{figures/QminJoint/train_H_Q_xCz_trnsf.png}
 \label{fig:qminjoint_train_H_Q_xCz}
  }%
\caption{{\color{red}PLACEHOLDER FIG}. 
Effect of the choice of $\mathfam{Q}_{Bob}$ for $\CHFbob{X}{Z}$ on: 
(a) Generalization gap for Alice's classifier; 
(b) Alice's test log likelihood;
(c) $\CHF{Y}{Z}$ of Bob's selected representation;
(d) $\CHFbob{X}{Z}$ of Bob's selected representation.
Each plot compares DIB with $\mathfam{Q}_{Alice} \subset \mathfam{Q}_{Bob}$ ($\mathfam{Q}^+$),$\mathfam{Q}_{Alice} = \mathfam{Q}_{Bob}$ ($\mathfam{Q}$),$\mathfam{Q}_{Bob} \subset \mathfam{Q}_{Alice}$ ($\mathfam{Q}^-$) DIB.
Note that the first term of DIB, $\CHF{Y}{Z}$, is always taken with respect to $\mathfam{Q}_{Alice} = \mathfam{Q}_{Bob}$.
}
\label{fig:qmin_joint}
\end{figure}

==> figures/QminJointVib/QminJointVib.tex <==
\begin{figure}
\centering
\subfloat[Generalization Gap]{
\includegraphics[width=.47\textwidth]{figures/QminJointVib/gap_loglike.png}
 \label{fig:qminjointvib_gap_loglike}
  }%
\subfloat[Test Loglike.]{
\includegraphics[width=.47\textwidth]{figures/QminJointVib/test_loglike.png}
 \label{fig:qminjointvib_test_loglike}
  }%
 \hfill
\subfloat[$\CHF{Y}{Z}$]{
\includegraphics[width=.47\textwidth]{figures/QminJointVib/train_H_Q_yCz_trnsf.png}
 \label{fig:qminjointvib_train_H_Q_yCz}
  }%
 \subfloat[Regularizer]{
\includegraphics[width=.47\textwidth]{figures/QminJointVib/superposed_star_bits.png}
 \label{fig:qminjointvib_train_H_Q_xCz}
  }%
\caption{{\color{red}PLACEHOLDER FIG}. 
Comparison between the DIB and VIB objective on: 
(a) Generalization gap for Alice's classifier; 
(b) Alice's test log likelihood;
(c) $\CHF{Y}{Z}$ of Bob's selected representation;
(d) The regularization term for Bob's selected representation.
}
\label{fig:qmin_joint_vib}
\end{figure}

==> figures/cifar10mnist/cifar10mnist.tex <==
\begin{figure}
\centering
\includegraphics[width=.47\textwidth]{figures/cifar10mnist/cifar10mnist.png}
\caption{Increasing $\beta$ not only increases the worst case performance but also decreases the amount of decodability of a distractor task.
}
\label{fig:cifar10mnist}
\end{figure}

==> figures/cifar10mnist/dataset.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/cifar10mnist/dataset.png}
    \caption{An illustration of the images in the CIFAR10+MNIST
    dataset that we use in the main paper. This dataset is similar
    to the one proposed in~\citep{AchilleS18dropout}. \textbf{L}:
    Denotes the original CIFAR10 label, while \textbf{D}: Denotes the distractor
    MNIST label.}
    \label{fig:cifar10_mnist_data}
\end{figure}

==> figures/reindexing/reindexing.tex <==
\begin{figure}
\centering
\subfloat[Generalization Gap]{
\includegraphics[width=.47\textwidth]{figures/reindexing/gap_loglike.png}
 \label{fig:reidx_gap_loglike}
  }%
\subfloat[Test Loglike.]{
\includegraphics[width=.47\textwidth]{figures/reindexing/test_loglike.png}
 \label{fig:reidx_test_loglike}
  }%
 \hfill
\subfloat[$\op{H_{\mathfam{Q}}}{\rv Y \cond \rv Z}$]{
\includegraphics[width=.47\textwidth]{figures/reindexing/train_H_Q_yCz_trnsf.png}
 \label{fig:reidx_train_H_Q_yCz}
  }%
 \subfloat[$\op{H_{\mathfam{Q}}}{\rv X \cond \rv Z}$]{
\includegraphics[width=.47\textwidth]{figures/reindexing/train_H_Q_xCz_trnsf.png}
 \label{fig:reidx_train_H_Q_xCz}
  }%
\caption{{\color{red}PLACEHOLDER FIG}. Effect of averaging over multiple selected indexing of $\mathcal{X}$. 
(a) Generalization gap for Alice's classifier; 
(b) Alice's test log likelihood;
(c) $\op{H_{\mathfam{Q}}}{\rv Y \cond \rv Z}$ of Bob's selected representation;
(d) $\op{H_{\mathfam{Q}}}{\rv X \cond \rv Z}$ of Bob's selected representation.
Each plot compares the DIB loss which uses [1,3,5,10,20] different indexing, and Fixed DIB loss which uses [1,3,5,10,20] different predictors for the \textit{same} indexing.
}
\label{fig:reindexing}
\end{figure}

==> figures/text/information_diag.tex <==
\begin{figure}[!t]
\centering

  
\begin{subfigure}[t]{0.32\linewidth}
\includegraphics[width=\linewidth]{figures/text/info_diag.jpg}
\subcaption{An information diagram
}
\end{subfigure} \hfill
\begin{subfigure}[t]{0.32\linewidth}
\includegraphics[width=\textwidth]{figures/text/stat_diag.jpg}
\subcaption{A statistic $\rv Z$ of $\rv X$}
\end{subfigure} \hfill
\begin{subfigure}[t]{0.32\linewidth}
\includegraphics[width=\textwidth]{figures/text/suff_diag.jpg}
\subcaption{$\rv Z$ is sufficient for $\rv Y$
}
\end{subfigure} 
\caption{The data processing inequality states that 
$\MI{Y}{Z} \leq \MI{Y}{X}$ for any statistic $\rv Z$ of $\rv X$ (middle plot).
$\rv Z$ is sufficient for $\rv Y$ if $\MI{Y}{Z} =\MI{Y}{X}$ (right plot).
To be minimal, it needs to be sufficient and have $\MI{X}{Z} =\MI{Y}{Z}$.}\label{fig:information_diag}
\end{figure}

==> text/dib.tex <==

In the previous section we proposed a measure of relevance of a random variable to predict an other one. We now consider how to use such formalism to learn an ``optimal'' representations $\rv Z$.

We will start by considering simplified version of the setting discussed in \cref{sec:problem_statement} through strong assumptions, which we will then gradually relax.



\subsection{$\mathfam{Q}$-Sufficiency}
\label{ssec:sufficiency}

In this subsection, we consider the case where both you and the downstream user (Alice) have access to the underlying probability measure $P_{\mathcal{X} \times \mathcal{Y}}$ instead of a training dataset. 
Furthermore, we assume that you both have access to a global optimizer.


In the well-posed setting, we would like to learn a representation which would yield the same expected loss as if we used the universal family $\universal{}$ and .

\begin{definition}[$\family{}$-Sufficient Statistic]\label{def:q-sufficiency}
A statistic $\rv Z$ of $\rv X$ is said predictive $\family{}$-sufficient for $\rv Y $ if $\CHF{y}{z} = \op{H}{\rv Y \cond \rv z}$. 
We denote the set of all such statistics $\Qsuff{}$.
\end{definition}

%The goal is to find a (if it exists) sufficient statistic, such that our predicitions would be as good as if the predictive family $\mathcal{Q}$ was not constrained.
Note that constraining $\family{}$ reduced the search space of possible statistics to chose from (empty in none realizable setting).


\begin{restatable}{proposition}{sufficiencies}\label{prop:sufficiencies}
Let $\family{}$, $\pFam{\mathcal{G}}$ be two predictive families. 
If $\family{} \subseteq \pFam{\mathcal{G}}$ then
$\Qsuff{} \subseteq \mathcal{S}_{\mathcal{G}}^{\rv Y \leftarrow \rv Z} \subseteq  \mathcal{S}_{\mathcal{U}}^{\rv Y \leftarrow \rv Z} = \suff{}$
\end{restatable}

Although, the previous proposition is very intuitive, it does raise an important question and suggests that current information based methods for representation learning and feature selection might not be useful. 
Indeed, previous work have proposed different ways of learning representations my maximizing the mutual information \cite{}. 
On the contrary \cref{prop:sufficiencies} shows that one can have a representation which is sufficient but not $\family{}$-sufficient for the prediction task at hand. 
For example, in the case of image classification, the input itself $\rv X$ is sufficient for $\rv Y$ but usually not $\family{}$-sufficient.
\yann{\textbf{@RAMA}: you had a pretty strong idea of what should be here, maybe you want to write that paragraph explaining that this is not an approximation but truly what we care about.}

%Contrary to sufficient statistics, a $\mathcal{Q}$ sufficent statistic might not always exist.

\subsection{Minimality and Generalization}
\label{ssec:minimality}

In practical settings, the optimization is never well-posed, i.e. we never have access to the underlying distribution but only samples from it. 
The typical way of dealing with this issue is by treating the empirical distribution $\hat{P}_{\rv X \times \rv Y}$ as the actual distribution.
I.e. we will recover $\family{}$-sufficient statistics for the empirical distribution. 
This raises an important question : how well will such statistic and its associated predictor \textit{generalize} to new samples from the underlying distribution ?
Are all $\family{}$-sufficient statistics equally good at generalizing ?

Intuitively, a statistic that generalizes well, is one from which a predictor would not be able to \textit{over-fit} the training data. 
I.e. it should not contain unnecessary information about $\hrv X$ that could be used by the downstream predictor. 
In the unconstrained case, this corresponds to a representation with low $\MI{X}{Z}$ (minimality \cref{def:predictive_min}).
Previous work have formalized this intuition by bounding the generalization gap by $\MI{X}{Z}$ \cite{shamir2010learning} or its empirical estimate \cite{vera2018role,rodriguez2019information}
\yann{Didn't go through this in detail but I think that what we propose also soves the issues raised by \cite{hafez2019compressed}}.
In the following, we posit that a large $\MI{X}{Z}$ would not yield to over-fitting, as long as this information can be decoded by the predictor. 
\yann{I really think we can get a bound which replaces entropy with predictive entropy in \cite{vera2018role} which would thus always be a tighter bound because predictive entropy is always smaller. This would make this paper much stronger.}
One issue for formalizing this notion is that $\family{}$ can generally not predict $\rv X$ ($\mathcal{X}$ and $\mathcal{Y}$ are usually different).
We instead have to consider a set of r.v. $\mathcal{N}$ that take values in $\mathcal{Y}$ but have the same information as $\rv X$.
%We formalize the notion of predictability of $\rv X$ by considering the predictability 
%that these bounds are very loose, as they do not take into account if such inform


%The set of minimal predictive $\family{}$-sufficient statistcs can also be written as a constrained optimization problem which does not depend on $\MI{X}{Z}$. 
%This is advantageous as mutual information is a notoriously hard term to estimate using an empirical distribution \citep{}.

\begin{restatable}[Minimal $\family{}$-Sufficient Statistic]{definition}{optimin}\label{def:q-min-sufficiency}
Let $\mathcal{T}$ be the set of all statistics of $\rv X$.
Let $\mathcal{N}$ be a (possibly uncountable) collection of statistics of $\rv X$ such that $\forall \rv N \in \mathcal{N}$ takes value in $\mathcal{Y} $ and there is a bijection between $\mathcal{N}$ and $\rv X$. 
Then we say that a  $\family{}$-sufficient statistic is minimal if it maximizes $\E{\rv N' \sim \mathrm{unif}(\mathcal{N})}{\CHF{ N'}{z}}$.
\end{restatable}

The previous definition has a very intuitive interpretation.
Let us illustrate it with the task of binary $32\times32$ black and white image classification of cats using the predictive family of logistic regressions from a 5 dimensional $\rv Z$ to $\hrv Y$.
A possible $\mathcal{N}$ would be the set of all binary labels that says whether a certain pixel takes value $i\in \{0,...,255\}$ ($\mathcal{N}$ contains 32*32*256 r.v.).
Let $\rv Z^{(1)}$ be the concatenation of the 5 first pixels,  $\rv Z^{(2)}$ the concatenation of 4 first pixels and the label, $\rv Z^{(3)}$ a 5-replicate of the label. 
$\rv Z^{(1)}$ would not be $\family{}$-sufficient as the 5 pixels are usually not sufficient to predict whether a cat is in the image
$\rv Z^{(2)}$ would be sufficient as it contains the label itself (which is linearly decodable) but not minimal as can help predicting the color of the pixels.

Such definition actually recover many useful measure in statistical learning theory.

\begin{restatable}[Links to Minimal $\family{}$-Sufficient Statistic]{proposition}{qminimallink}\label{def:q-min-link}
\begin{itemize}
\item \textbf{Rademacher Complexity} In the case of binary classification $\mathcal{Y}=\{0,1\}$, a minimal $\family{}$-sufficient statistic is a representation that would yield maximal training accuracy, while giving rise to minimal Rademacher complexity.
\item \textbf{Random Labeling} In the case of mutli label classification $\mathcal{Y}=\{0,1\}$, a minimal $\family{}$-sufficient statistic is a representation that would yield maximal training accuracy, while minimizing the ability of the functional class to fit randnom labels \cite{zhang2016understanding}.
\item \textbf{Minimal Sufficient Statistics} If $\family{} = \universal{}$ then a statistic $\rv Z$ is minimal $\family{}$-sufficient statistic if and only if it is minimal sufficient.
\end{itemize}
\end{restatable}

In addition to the link to these measure of complexity and its intuitive notion, one can also prove that the a minimal $\family{}$-sufficient statistic will provably generalize better. 




\begin{proof}
\yann{To write. But essentially : 1/ prove that sufficient iff $\op{H^{S}}{\rv Y \cond \rv Z} = \CHF{Y}{Z}$ due to strictly proper scoring rule. 2/ adding constant $\op{H^{S}}{\rv Y}$. 3/ Proving that minimal iff $\op{I}{\rv Y}{\rv X}=\MI{\rv Y}{\rv Z}$ due to data processing inequality (have to check for generalized) and independence. }
\end{proof}

\yann{I still have to write the link with generalization. Either I only cite previous work or prove generalization bounds on $\mathcal{Q}$-minimal sufficient statistics. As it is written now, it will probably not be much different than previous bounds. 
It can become very different (and very important) if we end up using minimizing something like $\DIF{T(\rv X)}{\rv X }$ (see the important discussion in the next subsection).
Concerning previous literature
\begin{description}
\item[Bounds using $\op{I}{T(\rv X);\rv X }$] These are the most important bounds for our work \cite{vera2018role,rodriguez2019information} . Note that \cite{hafez2019compressed} have an important part where they say that actually bounds are not applicable if learnign the encoder simultaneously.
\item[Bounds using $\op{I}{Q;\mathcal{D}}$] i.e. between data the selected Q by an algorithm \cite{russo2015much,jiao2017dependence,bu2019tightening}.
Essentially the bounds say that $\operatorname{gen}=O(\sqrt{\frac{2 \sigma^{2}}{N} I\left(\mathcal{D} ; Q\right)})$ where N is the sample size,and under the assumption that the loss
function L is $\sigma$-sub Gaussian, meaning it has a lighter tail than a Gaussian with variance $\sigma^2$.
\end{description}
}

\subsection{Highly Restricted $\mathcal{Q}$}

Using \cref{def:q-sufficiency} and \cref{def:q-min-sufficiency}, we can succinctly summarize the set of minimal sufficient statistics as the following constrained optimization problem. 

\begin{equation}\label{eqn:min_suff_ent}
\begin{aligned}
\Qsmin &= 
\arg \min_{Z \in \mathcal{T}} \quad \E{\rv N' \sim \mathrm{unif}(\mathcal{N})}{\CHF{ N'}{z}}  \\
& \textrm{s.t.} \quad  \CHF{Y}{z} =  \op{H}{\rv Y \cond \rv X}
\end{aligned}
\end{equation}

In the previous subsections, we focuses on the case where $\mathcal{Q}$-sufficent statistics exists.
Although this is is always the case for unrestricted predictive family \footnote{Even in the case where $\mathcal{Q}$-sufficent statistics exist, one might prefer to use the proposed relaxation to increase generalization capabilities at the expense of training error.}, it is generally not the case for $\mathcal{Q}$.
In such setting one can use the following relaxation.

\begin{definition}[$\mathcal{Q}$-Decodable Information Bottleneck]\label{def:diq}
The Lagrangian relaxation of \cref{eqn:min_suff_ent}.
\begin{equation}\label{eqn:min_suff_ent}
\mathcal{L}_{\mathcal{Q}IB} \eqdef \op{I^S}{T(\rv X);\rv X} - \beta \DIF{\rv Y}{\rv T(\rv X)}
\end{equation}
\end{definition}

Note that for $\mathcal{Q}=\Omega$ and log loss $S$ we recover the standard information bottleneck \cite{tishby2000information}.

\important{What we would really want is to replace $\op{I^S}{T(\rv X);\rv X}$ with something like $\DI{\mathrm{G}\circ\mathrm{Q}}{\rv X}{\rv T(\rv X)}$ as this:
\begin{enumerate}[noitemsep]
\item is provably easier to estimate. If we don't then we will have to use a variational estimate of $\op{I^S}{T(\rv X);\rv X}$ and then the practical impleemntation is that different from VIB (which does not work great). 
\item is very intuitive and I'm convince that this is what we care about for generalization (basically we do not care about the decreasing the information that Z has about X if the functional family cannot decode such information. I.e. if we are using linear decoders then all the non linear information about X is not important as Q will not ``have access to it'').
\end{enumerate}
The problems are the following:
\begin{enumerate}[noitemsep]
\item Have to find a definition that makes sense for minimality for which \cref{eqn:min_suff_ent} would still be a relaxation of a possibly different \cref{eqn:min_suff_ent}.
\item Have to be careful with the domain of $\mathcal{Q}$. For example one cannot use $\DIF{\rv Y}{\rv T(\rv X)}$ and $\DIF{\rv X}{\rv Z}$ because $\rv Z$ and $\rv X$ probably don't live in the same space.
\item We still want something like \cref{eqn:optimal_qib} because it is so intuitive. 
\end{enumerate}
If we do use something like $\DIF{\rv X}{\rv Z}$ then I need to have a deeper look into how to train both $p(z\cond x)$and $q(y \cond x)$. Until now I have been using joint training, which works pretty well, but I don't think this is the correct way of doing. Indeed we essentially have a minimax game like GANs and I would have to look deeper in the literature. I think I need to take gradients for each both separately. 
}

%\begin{itemize}[noitemsep]
%\item state the $\mathcal{Q}$-decodable information
%\item (IMPORTANT) separate I[X,Z] into a Q decodable and Q not decdable solution to show that it makes sense to minimize $I_Q[Z,X]$ only
%\end{itemize} 

\begin{restatable}{theorem}{optimalqib}
\yann{Still have to generalize to non log loss (KL divergence would be replaced with the corresponding divergence) + use the current notation.}
Given a Markov chain $\rv Y \to \rv X \to \rv Z$, the optimal encoder that minimizes $\mathcal{Q}$ decodable information bottleneck \cref{eqn:min_suff_ent} is

\begin{equation}\label{eqn:optimal_qib}
 p(z \cond x) = \frac{p(z)}{C(Y,x,\beta)}\exp \pa{- \beta \KL{p( Y \cond x), q(Y \cond z)}} 
\end{equation}

Where 

\begin{align}
q(\rv y \cond z) 
&\defeq \arg \inf _{q \in \mathcal{Q}} \mathbb{E}_{p(X, Y)}[-\log q(\rv y \cond z)] \label{eqn:q_yz} \\
p(z) &=  \mathbb{E}_{p(X)}[p(z \cond \rv x)] \label{eqn:p_z}
\end{align}

\end{restatable}

Refer to \cref{proof:qib} for the proof. 
Note that, this is a ``formal'' solution as the right hand side of \cref{eqn:q_yz} and \cref{eqn:p_z} depends on $ p(z \cond x)$ which depends itself on $p(z)$ and $q(\rv y \cond z)$.
The form of \cref{eqn:optimal_qib} is very intuitive, it states that the optimal encoder should find a $\rv Z$ such that $P_{\rv Y \cond \rv X}$ is close to $P_{\rv Y \cond \rv Z}$, i.e. predicting using the raw input or the representation should be the closest in the KL diveregnce sense.
\yann{If we were to draw similarities between rate-distortion theory, we would get that $\KL{p( Y \cond x), q(Y \cond z)}$ is the distortion measure, which is very appealing. Hopefully we can get that the S associated divergence is always the distortion measure.}

%\subsection{Generalization in Deep Learning}

\subsection{Optimization}

It simple problems we can find a good  $p(z \cond x)$ by extending the iterative Blahut-Arimoto algorithm to converge to a local optimal.

\begin{restatable}{theorem}{blahut}
\yann{Add details and and clean}
The minimization of \cref{eqn:DIF} can be done iteratively using the following equations until nothing changes:
$$\left\{\begin{array}{l}
{p_{t}(z | x)=\frac{p_{t}(z)}{C_t(Y,x,\beta)} \exp (- \beta \KL{p( Y \cond x), q_t(Y \cond z)}} \\
{p_{t+1}(z)=\int_{\rv X} p(x) p_{t}(z | x)} \\
{p_{t+1}(y | z)=\int_{\rv Y} p(y | x) p_{t}(x | z)} \\
{q_{t+1}(y | z)=\arg \min_{q \in \mathcal{Q}} \int_{\rv Y} \KL{ p_{t+1}(y | z), q(y | z)} }
\end{array}\right.$$
\end{restatable}


For real world applications with continuous random variable would usually we will directly minimize the $\mathcal{Q}$-Decodable Information jointly with respect to $p(z \cond x)$ and $q(\rv y \cond z)$ .



==> text/dif.tex <==

\begin{definition}[Predictive Family]\label{def:predictive}
A predictive family of $\rv Y$ given $\rv Z$, denoted $\mathfam{Q} \subseteq \mathcal{P}(\mathcal{Y} | \mathcal{Z})$, is a collection of probabilistic predictors $\pred{}$  that are
\begin{inlinelist}
\item invariant to permutations of $\mathcal{Y}$;
\item can predict the true marginal regardless of the input, i.e. $\exists \pred{} \in  \mathfam{Q}$ s.t. $\forall P_{\rv Y} \in \mathcal{P}(\mathcal{Y}), \ \forall z \in \mathcal{Z}, \  \predS{} = P_{\rv Y}$.
\end{inlinelist}
We will refer to the largest such family $\universal{} \defeq \mathcal{P}(\mathcal{Y}|\mathcal{Z}) $ as the  \textit{universal} one and use $q(y|z)$ as a shorthand for $\predS{}(y)$.\footnote{We use the notation of regular conditional probabilities for probabilistic predictors as both are equivalent. We use the notation of probability mass functions, since we assume finite sample spaces.}
\end{definition}

\ydnote{Maybe this definition could go in the previous section as Stefano also needs such a definition. But it's important to point out that ours is more restrictive (but always holds because we assumed finite sample spaces). It's just more clear to talk about that}

In the classification setting we are considering, both assumptions hold for most predictive families that frequently used in ML, e.g. linear classifiers, decision trees, or neural networks.  
The first requirement is trivial and simply says that the labeling convention does not matter. 
The second requirement is typically achievable by setting all the parameters of a model to zero besides the biases.  
\footnote{The assumptions we use are stronger than in \cite{xu2020theory}. Loosening these requirements is important when dealing with continuous r.v.s. While we can also extend our framework to this setting, we chose not to for clarity.}



In the previous section, we discussed a recent generalization of mutual information that considers to predictive family of interest $\family{}$ \cite{xu2020theory}. This can be used to quantify the information that a representation $\rv Z$ has about the target $\rv Y$ from the perspective of $\family{} : \mathcal{Z} \to \mathcal{Y}$ but it cannot generally be used to quantify the information that $\rv Z$ has about the input $\rv X$ as the sample space $\mathcal{X}$ is not necessarily equal to that of  $\mathcal{Y}$.
To circumvent this problem, we will decompose the r.v. $\rv X$ in a collection of random variables $\{\rv N_i\}_i$ such that each $\rv N_i$ t.v.i $\mathcal{Y}$ to ensure that $q_{n_i|z}$ is well-defined.
This decomposition has to satisfy the following key properties
\footnote{This decomposition is related to the notion of strong decomposition of random variables in probability theory \cite{hoffmann2007strong}, in that it requires every element $\rv N_i$ to be non degenerate and independent. 
The main differences being that we constrain the sample space of each member of the decomposition to $\mathcal{Y}$, and that we replaced the requiremnt of decomposing random variables in a sum of other random variables by the bijective property.  
}
:


\begin{definition}[$\mathcal{Y}$ Decomposition of Random Variables]\label{def:decomp}
A collection of r.v. $\rv N=\{\rv N_i\}_i$ are a $\mathcal{Y}$ decomposition of  $\rv X$.
If 
\begin{itemize}
\item \textbf{Take value in $\mathcal{Y}$}. Each $\rv N_i \in \rv N$ t.v.i in $\mathcal{Y}$ \ydnote{actually in a set whose support is a subset of $\mathcal{Y}$ }. 
\item \textbf{Bijection} There exists a bijection $f$ s.t. $\rv X = f(\rv N)$;
\item \textbf{Independence} $\rv N_i \perp \rv N_j, \ \forall \rv N_i \in \rv N \neq \rv N_j \in \rv N$.
%\item \textbf{Not Constant} There are no degenerate r.v. $\rv N_i$. \ydnote{This is not really used as the entropy and decodable entropy will always be 0 in that case so we can remove all the degnerate r.v., but }
\end{itemize}
\end{definition}

Armed with a set of decomposed random variables that take value in the correct sample space, we can define the notion of $\mathfam{Q}$-\textit{decodable information} as follows.

\begin{restatable}[$\mathfam{Q}$-Decodable Information]{definition}{decentropy}\label{def:q_entropy}
The decodable entropy of $\rv X$ t.v.i $\mathcal{X}$  conditioned on $\rv Z$ with respect to $\family{} \subseteq \mathcal{P}{(\mathcal{Y} | \mathcal{Z})}$ (where $\mathcal{X}$ is not necessarily $\mathcal{Y}$) and $\rv N$ a $\mathcal{Y}$ decomposition of $\rv X$, is \ydnote{Will most probably have to takes expectation over all decompositions, but keeping this } :
\[
\CHF{X}{z} 
\defeq \sum_{N_i \in N}  \inf_{Q \in \mathfam{Q}} \E{n_i,z \sim P_{\rv N_i \times \rv z}}{- \log q(n_i \cond z)}
\]
The associated decodable information is 
\[
\DIF{X}{Z} \defeq \op{H}{\rv X} - \CHF{X}{z} 
\]
\end{restatable}

The decodable information measures the difference in expected log loss between predicting a r.v. using its marginal entropy $P_{\rv X}$ or by decomposing it into meaningful components and using the best possible predictor in a functional family $\mathfam{Q}$ on top of $\rv Z$ to predict each component.
It intuively considers the amount of information that $\mathfam{Q}$ can \textit{decode} (extract) from a given input $\rv Z$.
The decodable information enjoys some desirable properties for representation learning. Namely, that using a larger predictive family increases the amount of information that can be decoded, that it is non-negative, and equal to zero if two random variables are independent as there is no information to decode.


\begin{restatable}[Properties of Decodable Entropy]{proposition}{propentropy}\label{prop:properties}

Let $\mathfam{Q} \subseteq \PYZ{} $, $\mathfam{G} \subseteq \PYZ{}$ denote two predictive families,  and  $\rv X$ t.v.i an arbitrary $\mathcal{X}$, while $\rv Z$ $\rv Y$ respectively t.v.i in the domain $\mathcal{Z}$ and codomain $\mathcal{Y}$ of the predictive families, then
\begin{itemize}
\item \textbf{Monotonicity} If $\mathfam{Q} \subseteq \mathfam{G}$ then $\DIF{X}{Z} \geq \DI{\mathfam{G}}{X}{Z}$.
\item \textbf{Independence} If $\rv X \perp \rv z $ then $\DIF{X}{Z} = 0$.
\item \textbf{Non Negativity} $\DIF{X}{Z} \geq 0$.
\end{itemize}
\end{restatable}

In addition we can show that the decodable information recovers the mutual information when $\mathfam{Q}=\mathfam{U}$ and generalizes the notion of $\mathfam{V}$-information when the sample space of the random variable of interest is the codomain of the predictive family.

\begin{restatable}[Special Cases]{proposition}{specialcase}\label{prop:special_cases}
Let $\rv Y, \rv X, \rv Z$ be such as in  \cref{prop:properties} and  $\mathfam{U} \defeq \PYZ{}$ be the universal predictive family, then
\begin{itemize}
    \item \textbf{Mutual Information} 
$\DI{\mathfam{U}}{X}{Z} = \MI{X}{Z}$ regardless of the sample space $\mathfam{X}$. 
    \item \textbf{$\mathfam{V}$-information} 
$\DI{\mathfam{Q}}{Y}{Z} = \vI{Y}{Z}$ for $\rv Y$, where $\mathfam{V}=\mathfam{Q}$.
\end{itemize}
\end{restatable}
 
\ydnote{I removed Base b expansion from here, because I think it makes more sense to talk about it in the section about estimation and optimization as it is now an approximation to what we want, and the reader will probably first want to see what we do with it}


Importantly, the decodable entropy does not satisfy the data processing inequality nor the invariance to bijections, which we argue against in \cref{sec:information_theory}. 
In contrast to conditional entropy, decodable information can thus formalize the usefulness of the kernel trick and deep encoders as complex transformations that increase linearly decodable information.
Although the measure satisfies some properties that seem interesting, its usefulness really come from the theory that we develop in the following sections.
Namely that ``optimal'' representations $\rv Z^*$ that allows for minimal test loss while ensuring minimal generalization gap can be learned by maximizing  $\DIF{Y}{Z}$ while minimizing $\DIF{X}{Z}$.
In analogy to minimal sufficient representations \cref{eqn:min_suff_ent} we will call such representation $\mathfam{Q}$-minimal $\mathfam{Q}$-sufficient :


We will prove our claims and support themooolgcdxxouyp empirically by considering simplified version of the setting discussed in \cref{sec:formal_prob_state} through strong assumptions, which we will then gradually relax.

